Measurements of top-quark pair spin correlations in the $e\mu$ channel at $\sqrt{s} = 13$ TeV using $pp$ collisions in the ATLAS detector

A measurement of observables sensitive to spin correlations in $t\bar{t}$ production is presented, using 36.1 fb$^{-1}$ of $pp$ collision data at $\sqrt{s} = 13$ TeV recorded with the ATLAS detector at the Large Hadron Collider. Differential cross-sections are measured in events with exactly one electron and one muon with opposite-sign electric charge as a function of the azimuthal opening angle and the absolute difference in pseudorapidity between the electron and muon candidates in the laboratory frame. The azimuthal opening angle is also measured as a function of the invariant mass of the $t\bar{t}$ system. The measured differential cross-sections are compared to predictions by several NLO Monte Carlo generators and fixed-order calculations. The observed degree of spin correlation is somewhat higher than predicted by the generators used. The data are consistent with the prediction of one of the fixed-order calculations at NLO, but agree less well with higher-order predictions. Using these leptonic observables, a search is performed for pair production of supersymmetric top squarks decaying into Standard Model top quarks and light neutralinos. Top squark masses between 170 and 230 GeV are largely excluded at the 95% confidence level for kinematically allowed values of the neutralino mass.

==> tables/full_systematics_dphi_ll_parton_normalised.tex <==
\begin{table}
\caption{Full list of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude.}
\scriptsize
\centering
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.1  &  0.1 -- 0.2  &  0.2 -- 0.3  &  0.3 -- 0.4  &  0.4 -- 0.5  &  0.5 -- 0.6  &  0.6 -- 0.7  &  0.7 -- 0.8  &  0.8 -- 0.9  &  0.9 -- 1.0 \\ 
\midrule 
Source & \multicolumn{10}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
nlo &  & $^{0.0789}_{0.0} $ & $^{-0.3543}_{0.0} $ & $^{-1.6558}_{0.0} $ & $^{0.4442}_{0.0} $ & $^{-0.4083}_{0.0} $ & $^{1.6654}_{0.0} $ & $^{0.6554}_{0.0} $ & $^{-0.3804}_{0.0} $ & $^{0.2548}_{0.0} $ & $^{-0.4512}_{0.0} $ \\ 
pdf pdf4lhc 30 &  & $^{0.2689}_{0.0} $ & $^{0.2779}_{0.0} $ & $^{0.26}_{0.0} $ & $^{0.2043}_{0.0} $ & $^{0.1195}_{0.0} $ & $^{0.044}_{0.0} $ & $^{0.0661}_{0.0} $ & $^{0.1805}_{0.0} $ & $^{0.2904}_{0.0} $ & $^{0.3732}_{0.0} $ \\ 
shower &  & $^{0.2475}_{0.0} $ & $^{-0.4345}_{0.0} $ & $^{0.109}_{0.0} $ & $^{0.1627}_{0.0} $ & $^{0.0489}_{0.0} $ & $^{-0.5896}_{0.0} $ & $^{-0.6565}_{0.0} $ & $^{0.5985}_{0.0} $ & $^{0.328}_{0.0} $ & $^{0.0879}_{0.0} $ \\ 
rad  &  & $^{2.1792}_{1.4776}$ & $^{-0.5746}_{1.0245}$ & $^{1.5255}_{1.2149}$ & $^{1.3837}_{0.2871}$ & $^{0.1682}_{0.2152}$ & $^{-0.2431}_{0.3055}$ & $^{-1.7634}_{-0.7256}$ & $^{-0.2036}_{-1.689}$ & $^{-0.2027}_{-0.5516}$ & $^{-1.3475}_{-0.625}$ \\ 
Wt xsec  &  & $^{-0.0016}_{0.0016}$ & $^{0.0013}_{-0.0012}$ & $^{-0.0078}_{0.0078}$ & $^{0.0017}_{-0.0017}$ & $^{-0.0024}_{0.0024}$ & $^{-0.002}_{0.002}$ & $^{0.0069}_{-0.0068}$ & $^{0.0022}_{-0.0022}$ & $^{-0.003}_{0.003}$ & $^{0.0032}_{-0.0032}$ \\ 
Wt xsec shape &  & $^{-0.1363}_{0.0} $ & $^{-0.1959}_{0.0} $ & $^{-0.0335}_{0.0} $ & $^{-0.0215}_{0.0} $ & $^{0.0347}_{0.0} $ & $^{0.0338}_{0.0} $ & $^{-0.0951}_{0.0} $ & $^{0.036}_{0.0} $ & $^{0.1303}_{0.0} $ & $^{0.1504}_{0.0} $ \\ 
Ztau xsec  &  & $^{-0.0103}_{0.0103}$ & $^{-0.0063}_{0.0063}$ & $^{-0.0081}_{0.0081}$ & $^{-0.0103}_{0.0103}$ & $^{-0.0059}_{0.0059}$ & $^{-0.0036}_{0.0036}$ & $^{0.0074}_{-0.0074}$ & $^{0.006}_{-0.006}$ & $^{0.0108}_{-0.0108}$ & $^{0.0112}_{-0.0112}$ \\ 
db xsec  &  & $^{-0.0076}_{0.0076}$ & $^{-0.0063}_{0.0063}$ & $^{-0.0033}_{0.0033}$ & $^{-0.0018}_{0.0018}$ & $^{-0.0003}_{0.0003}$ & $^{0.0028}_{-0.0028}$ & $^{0.0033}_{-0.0033}$ & $^{0.0026}_{-0.0026}$ & $^{0.0022}_{-0.0022}$ & $^{0.0044}_{-0.0044}$ \\ 
fake xsec  &  & $^{-0.0331}_{0.0335}$ & $^{0.0025}_{-0.0026}$ & $^{-0.0044}_{0.0044}$ & $^{0.0257}_{-0.026}$ & $^{0.0378}_{-0.0383}$ & $^{-0.0014}_{0.0014}$ & $^{0.0088}_{-0.0089}$ & $^{0.0159}_{-0.0161}$ & $^{-0.0274}_{0.0277}$ & $^{-0.0197}_{0.02}$ \\ 
fake xsec shape &  & $^{-0.0869}_{0.0} $ & $^{0.0032}_{0.0} $ & $^{0.1722}_{0.0} $ & $^{-0.3711}_{0.0} $ & $^{-0.1864}_{0.0} $ & $^{0.1404}_{0.0} $ & $^{0.0432}_{0.0} $ & $^{0.199}_{0.0} $ & $^{-0.0254}_{0.0} $ & $^{0.0527}_{0.0} $ \\ 
Zjts xsec  &  & $^{-0.0231}_{0.0231}$ & $^{-0.0141}_{0.0141}$ & $^{-0.0181}_{0.0181}$ & $^{-0.0232}_{0.0232}$ & $^{-0.0133}_{0.0133}$ & $^{-0.0081}_{0.0081}$ & $^{0.0166}_{-0.0166}$ & $^{0.0135}_{-0.0135}$ & $^{0.0243}_{-0.0243}$ & $^{0.0251}_{-0.0251}$ \\ 
ttV xsec  &  & $^{0.0}_{0.0} $ & $^{-0.0007}_{0.0007}$ & $^{-0.0014}_{0.0014}$ & $^{0.0007}_{-0.0007}$ & $^{0.001}_{-0.001}$ & $^{-0.0005}_{0.0005}$ & $^{0.0006}_{-0.0006}$ & $^{0.0}_{0.0} $ & $^{0.0002}_{-0.0002}$ & $^{0.0}_{0.0} $ \\ 
tWZ xsec  &  & $^{0.0}_{0.0002}$ & $^{-0.0002}_{0.0005}$ & $^{0.0}_{-0.0002}$ & $^{0.0}_{0.0002}$ & $^{0.0}_{0.0002}$ & $^{0.0}_{-0.0001}$ & $^{-0.0002}_{0.0004}$ & $^{0.0}_{0.0} $ & $^{0.0}_{-0.0002}$ & $^{0.0002}_{-0.0007}$ \\ 
tttt xsec  &  & $^{-0.0008}_{0.0008}$ & $^{-0.0006}_{0.0006}$ & $^{-0.0005}_{0.0005}$ & $^{-0.0003}_{0.0003}$ & $^{0.0}_{0.0} $ & $^{0.0001}_{-0.0001}$ & $^{0.0}_{0.0} $ & $^{0.0004}_{-0.0004}$ & $^{0.0005}_{-0.0005}$ & $^{0.0006}_{-0.0006}$ \\ 
ttWW xsec  &  & $^{-0.0008}_{0.0008}$ & $^{-0.0003}_{0.0003}$ & $^{-0.0002}_{0.0002}$ & $^{-0.0001}_{0.0001}$ & $^{-0.0002}_{0.0002}$ & $^{-0.0002}_{0.0002}$ & $^{0.0003}_{-0.0003}$ & $^{0.0004}_{-0.0004}$ & $^{0.0004}_{-0.0004}$ & $^{0.0004}_{-0.0004}$ \\ 
tZ xsec  &  & $^{-0.0001}_{0.0001}$ & $^{-0.0009}_{0.0009}$ & $^{-0.0011}_{0.0011}$ & $^{-0.0005}_{0.0005}$ & $^{-0.0004}_{0.0004}$ & $^{0.0004}_{-0.0004}$ & $^{0.0007}_{-0.0007}$ & $^{0.0001}_{-0.0001}$ & $^{0.0005}_{-0.0005}$ & $^{0.0006}_{-0.0006}$ \\ 
ttgam xsec  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
ttH xsec  &  & $^{-0.0021}_{0.003}$ & $^{-0.0012}_{0.0018}$ & $^{-0.0007}_{0.001}$ & $^{-0.0002}_{0.0003}$ & $^{0.0002}_{-0.0003}$ & $^{0.0004}_{-0.0006}$ & $^{0.0004}_{-0.0006}$ & $^{0.0006}_{-0.0009}$ & $^{0.0007}_{-0.001}$ & $^{0.001}_{-0.0014}$ \\ 
pileup  &  & $^{0.2885}_{-0.0743}$ & $^{-0.2871}_{0.2673}$ & $^{-0.2914}_{0.3232}$ & $^{-0.1015}_{0.1079}$ & $^{-0.0332}_{0.0412}$ & $^{-0.2745}_{0.0963}$ & $^{0.1522}_{-0.1207}$ & $^{0.1098}_{-0.0764}$ & $^{0.0024}_{-0.0943}$ & $^{0.3136}_{-0.3091}$ \\ 
lumi  &  & $^{0.0099}_{-0.0103}$ & $^{0.0047}_{-0.0049}$ & $^{0.0082}_{-0.0086}$ & $^{0.0028}_{-0.003}$ & $^{0.0013}_{-0.0013}$ & $^{0.0013}_{-0.0014}$ & $^{-0.0075}_{0.0079}$ & $^{-0.0053}_{0.0055}$ & $^{-0.0029}_{0.003}$ & $^{-0.0067}_{0.007}$ \\ 
leptonSF EL SF Trigger  &  & $^{0.0074}_{-0.0074}$ & $^{0.0068}_{-0.0068}$ & $^{0.006}_{-0.006}$ & $^{0.0043}_{-0.0043}$ & $^{0.002}_{-0.002}$ & $^{-0.0004}_{0.0004}$ & $^{-0.0025}_{0.0025}$ & $^{-0.0044}_{0.0044}$ & $^{-0.0065}_{0.0065}$ & $^{-0.0068}_{0.0068}$ \\ 
leptonSF EL SF Reco  &  & $^{-0.002}_{0.002}$ & $^{-0.0027}_{0.0027}$ & $^{-0.0041}_{0.0041}$ & $^{-0.0035}_{0.0035}$ & $^{-0.0045}_{0.0045}$ & $^{-0.0035}_{0.0035}$ & $^{-0.0012}_{0.0012}$ & $^{0.0015}_{-0.0015}$ & $^{0.0064}_{-0.0064}$ & $^{0.009}_{-0.009}$ \\ 
leptonSF EL SF ID  &  & $^{-0.0124}_{0.0126}$ & $^{-0.0201}_{0.0204}$ & $^{-0.0261}_{0.0265}$ & $^{-0.0266}_{0.027}$ & $^{-0.0303}_{0.0308}$ & $^{-0.0241}_{0.0245}$ & $^{-0.0119}_{0.0121}$ & $^{0.0086}_{-0.0088}$ & $^{0.0454}_{-0.0461}$ & $^{0.0664}_{-0.0675}$ \\ 
leptonSF EL SF Isol  &  & $^{-0.0417}_{0.0419}$ & $^{-0.0435}_{0.0436}$ & $^{-0.0448}_{0.045}$ & $^{-0.0409}_{0.041}$ & $^{-0.0363}_{0.0364}$ & $^{-0.0269}_{0.027}$ & $^{-0.0101}_{0.0101}$ & $^{0.0191}_{-0.0192}$ & $^{0.0659}_{-0.0662}$ & $^{0.1054}_{-0.1058}$ \\ 
leptonSF MU SF Trigger STAT  &  & $^{0.0093}_{-0.0094}$ & $^{0.0091}_{-0.0092}$ & $^{0.007}_{-0.0071}$ & $^{0.0056}_{-0.0057}$ & $^{0.0031}_{-0.0031}$ & $^{-0.0001}_{0.0001}$ & $^{-0.0032}_{0.0032}$ & $^{-0.0057}_{0.0058}$ & $^{-0.0077}_{0.0078}$ & $^{-0.0097}_{0.0099}$ \\ 
leptonSF MU SF Trigger SYST  &  & $^{0.019}_{-0.0186}$ & $^{0.0175}_{-0.0171}$ & $^{0.0129}_{-0.0126}$ & $^{0.0102}_{-0.01}$ & $^{0.0058}_{-0.0057}$ & $^{0.0003}_{-0.0003}$ & $^{-0.0062}_{0.0061}$ & $^{-0.0109}_{0.0106}$ & $^{-0.0156}_{0.0153}$ & $^{-0.0181}_{0.0178}$ \\ 
leptonSF MU SF ID STAT  &  & $^{0.0002}_{-0.0002}$ & $^{0.0015}_{-0.0015}$ & $^{0.0002}_{-0.0002}$ & $^{0.0001}_{-0.0001}$ & $^{0.0002}_{-0.0002}$ & $^{0.0005}_{-0.0005}$ & $^{-0.0003}_{0.0003}$ & $^{0.0}_{0.0} $ & $^{-0.0008}_{0.0008}$ & $^{-0.001}_{0.001}$ \\ 
leptonSF MU SF ID SYST  &  & $^{-0.0365}_{0.0367}$ & $^{-0.0401}_{0.0404}$ & $^{-0.0377}_{0.038}$ & $^{-0.0353}_{0.0356}$ & $^{-0.0296}_{0.0299}$ & $^{-0.019}_{0.0191}$ & $^{-0.0066}_{0.0067}$ & $^{0.0236}_{-0.0238}$ & $^{0.0547}_{-0.0551}$ & $^{0.0814}_{-0.0819}$ \\ 
leptonSF MU SF ID STAT LOWPT  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
leptonSF MU SF ID SYST LOWPT  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
leptonSF MU SF Isol STAT  &  & $^{-0.0019}_{0.0019}$ & $^{-0.0021}_{0.0021}$ & $^{-0.0019}_{0.0019}$ & $^{-0.0018}_{0.0018}$ & $^{-0.0016}_{0.0016}$ & $^{-0.0011}_{0.0011}$ & $^{-0.0003}_{0.0003}$ & $^{0.0011}_{-0.0011}$ & $^{0.0029}_{-0.0029}$ & $^{0.0043}_{-0.0043}$ \\ 
leptonSF MU SF Isol SYST  &  & $^{0.0013}_{-0.0013}$ & $^{0.0008}_{-0.0008}$ & $^{0.001}_{-0.001}$ & $^{0.0003}_{-0.0003}$ & $^{0.0}_{0.0} $ & $^{-0.0003}_{0.0003}$ & $^{-0.0012}_{0.0012}$ & $^{-0.0009}_{0.0009}$ & $^{-0.0003}_{0.0003}$ & $^{0.0}_{0.0} $ \\ 
leptonSF MU SF TTVA STAT  &  & $^{0.0002}_{-0.0002}$ & $^{0.0}_{0.0} $ & $^{0.0004}_{-0.0004}$ & $^{0.0}_{0.0} $ & $^{-0.0001}_{0.0001}$ & $^{0.0}_{0.0} $ & $^{-0.0002}_{0.0002}$ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{-0.0002}_{0.0002}$ \\ 
leptonSF MU SF TTVA SYST  &  & $^{-0.0009}_{0.0009}$ & $^{-0.0015}_{0.0015}$ & $^{0.0002}_{-0.0002}$ & $^{-0.0006}_{0.0006}$ & $^{-0.0013}_{0.0013}$ & $^{0.0003}_{-0.0003}$ & $^{0.0008}_{-0.0008}$ & $^{0.0005}_{-0.0005}$ & $^{0.0005}_{-0.0005}$ & $^{0.0011}_{-0.0011}$ \\ 
weight jvt  &  & $^{0.008}_{-0.0092}$ & $^{0.0167}_{-0.0165}$ & $^{0.0094}_{-0.0096}$ & $^{0.0074}_{-0.0072}$ & $^{0.003}_{-0.0033}$ & $^{0.0072}_{-0.0066}$ & $^{-0.0046}_{0.0051}$ & $^{-0.0217}_{0.0205}$ & $^{-0.0038}_{0.0047}$ & $^{-0.0112}_{0.0116}$ \\ 
weight bTagSF 77 eigenvars B 0 &  & $^{0.0193}_{-0.0165}$ & $^{0.025}_{-0.0215}$ & $^{0.0226}_{-0.0229}$ & $^{-0.0026}_{0.0048}$ & $^{0.0076}_{-0.0078}$ & $^{0.0154}_{-0.0161}$ & $^{0.0005}_{-0.0017}$ & $^{-0.0037}_{0.0019}$ & $^{-0.0265}_{0.0262}$ & $^{-0.0374}_{0.0349}$ \\ 
weight bTagSF 77 eigenvars B 1 &  & $^{-0.011}_{0.0116}$ & $^{0.0198}_{-0.0194}$ & $^{0.005}_{-0.0046}$ & $^{0.0057}_{-0.0053}$ & $^{-0.0047}_{0.005}$ & $^{0.0103}_{-0.0103}$ & $^{0.0033}_{-0.0034}$ & $^{0.0017}_{-0.002}$ & $^{-0.01}_{0.0095}$ & $^{-0.0142}_{0.0136}$ \\ 
weight bTagSF 77 eigenvars B 2 &  & $^{0.034}_{-0.0345}$ & $^{0.0219}_{-0.0223}$ & $^{0.0175}_{-0.018}$ & $^{0.0228}_{-0.0231}$ & $^{0.0115}_{-0.0117}$ & $^{-0.0047}_{0.0046}$ & $^{-0.0128}_{0.0129}$ & $^{-0.0256}_{0.026}$ & $^{-0.0198}_{0.0203}$ & $^{-0.0222}_{0.0227}$ \\ 
weight bTagSF 77 eigenvars B 3 &  & $^{0.0002}_{-0.0002}$ & $^{-0.0058}_{0.0058}$ & $^{-0.0013}_{0.0014}$ & $^{-0.0033}_{0.0033}$ & $^{0.0015}_{-0.0015}$ & $^{0.0032}_{-0.0033}$ & $^{0.0014}_{-0.0014}$ & $^{0.0006}_{-0.0006}$ & $^{0.0008}_{-0.0008}$ & $^{0.0012}_{-0.0012}$ \\ 
weight bTagSF 77 eigenvars B 4 &  & $^{-0.0068}_{0.0068}$ & $^{-0.0043}_{0.0043}$ & $^{-0.0053}_{0.0053}$ & $^{-0.0026}_{0.0026}$ & $^{-0.0025}_{0.0025}$ & $^{-0.0002}_{0.0002}$ & $^{0.0035}_{-0.0035}$ & $^{0.0039}_{-0.0039}$ & $^{0.0042}_{-0.0042}$ & $^{0.0054}_{-0.0054}$ \\ 
weight bTagSF 77 eigenvars B 5 &  & $^{0.0009}_{-0.0009}$ & $^{0.0006}_{-0.0006}$ & $^{0.0004}_{-0.0004}$ & $^{0.0003}_{-0.0003}$ & $^{0.0003}_{-0.0003}$ & $^{0.0}_{0.0} $ & $^{-0.0004}_{0.0004}$ & $^{-0.0004}_{0.0004}$ & $^{-0.0005}_{0.0005}$ & $^{-0.0007}_{0.0007}$ \\ 
weight bTagSF 77 eigenvars C 0 &  & $^{-0.0128}_{0.013}$ & $^{0.0007}_{-0.0007}$ & $^{-0.0113}_{0.0112}$ & $^{0.0055}_{-0.0056}$ & $^{-0.0036}_{0.0036}$ & $^{-0.0026}_{0.0026}$ & $^{0.0062}_{-0.0061}$ & $^{0.0036}_{-0.0036}$ & $^{0.0066}_{-0.0066}$ & $^{0.0028}_{-0.0028}$ \\ 
weight bTagSF 77 eigenvars C 1 &  & $^{-0.0029}_{0.0029}$ & $^{-0.0016}_{0.0017}$ & $^{-0.0114}_{0.0114}$ & $^{-0.0007}_{0.0006}$ & $^{0.0021}_{-0.0021}$ & $^{0.0023}_{-0.0023}$ & $^{-0.0003}_{0.0003}$ & $^{0.0029}_{-0.0029}$ & $^{0.0043}_{-0.0043}$ & $^{0.002}_{-0.002}$ \\ 
weight bTagSF 77 eigenvars C 2 &  & $^{-0.0021}_{0.0021}$ & $^{-0.0007}_{0.0008}$ & $^{-0.006}_{0.006}$ & $^{0.002}_{-0.002}$ & $^{-0.0011}_{0.0011}$ & $^{0.0003}_{-0.0003}$ & $^{0.0018}_{-0.0018}$ & $^{0.002}_{-0.002}$ & $^{0.002}_{-0.002}$ & $^{0.0002}_{-0.0002}$ \\ 
weight bTagSF 77 eigenvars C 3 &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
weight bTagSF 77 eigenvars Light 0 &  & $^{-0.0239}_{0.0216}$ & $^{-0.0112}_{0.0098}$ & $^{0.0138}_{-0.0138}$ & $^{-0.0124}_{0.0152}$ & $^{0.0031}_{-0.0044}$ & $^{-0.0176}_{0.0166}$ & $^{0.0154}_{-0.0155}$ & $^{0.0218}_{-0.0206}$ & $^{-0.0054}_{0.0065}$ & $^{0.0084}_{-0.0083}$ \\ 
weight bTagSF 77 eigenvars Light 1 &  & $^{-0.0009}_{0.0007}$ & $^{0.0022}_{-0.0024}$ & $^{-0.0094}_{0.0094}$ & $^{0.0005}_{0.0} $ & $^{-0.0023}_{0.0021}$ & $^{0.0091}_{-0.0092}$ & $^{-0.0049}_{0.0049}$ & $^{-0.0044}_{0.0045}$ & $^{0.006}_{-0.0058}$ & $^{0.0024}_{-0.0025}$ \\ 
weight bTagSF 77 eigenvars Light 2 &  & $^{-0.027}_{0.027}$ & $^{-0.0096}_{0.0096}$ & $^{-0.0273}_{0.0271}$ & $^{-0.0189}_{0.0185}$ & $^{-0.0021}_{0.0017}$ & $^{0.0187}_{-0.0182}$ & $^{0.0009}_{-0.0004}$ & $^{0.007}_{-0.0069}$ & $^{0.0166}_{-0.0164}$ & $^{0.0238}_{-0.0242}$ \\ 
weight bTagSF 77 eigenvars Light 3 &  & $^{-0.0162}_{0.0163}$ & $^{-0.0066}_{0.0067}$ & $^{-0.0145}_{0.0145}$ & $^{-0.0116}_{0.0113}$ & $^{0.0006}_{-0.0007}$ & $^{0.0088}_{-0.0086}$ & $^{0.0014}_{-0.0012}$ & $^{0.0058}_{-0.0057}$ & $^{0.0083}_{-0.0084}$ & $^{0.0137}_{-0.0138}$ \\ 
weight bTagSF 77 eigenvars Light 4 &  & $^{0.0057}_{-0.0057}$ & $^{-0.0038}_{0.0039}$ & $^{0.0113}_{-0.0109}$ & $^{-0.0008}_{0.0011}$ & $^{-0.0187}_{0.0185}$ & $^{0.0006}_{-0.0009}$ & $^{0.0064}_{-0.0066}$ & $^{-0.0032}_{0.0032}$ & $^{0.0006}_{-0.0003}$ & $^{0.0025}_{-0.0026}$ \\ 
weight bTagSF 77 eigenvars Light 5 &  & $^{0.0016}_{-0.0016}$ & $^{0.0036}_{-0.0037}$ & $^{0.0022}_{-0.0022}$ & $^{0.0029}_{-0.0029}$ & $^{-0.0047}_{0.0047}$ & $^{0.0019}_{-0.0019}$ & $^{-0.0018}_{0.0018}$ & $^{-0.0034}_{0.0034}$ & $^{0.0013}_{-0.0012}$ & $^{-0.0019}_{0.0019}$ \\ 
weight bTagSF 77 eigenvars Light 6 &  & $^{0.0002}_{-0.0002}$ & $^{0.0019}_{-0.0019}$ & $^{0.0}_{0.0} $ & $^{0.0018}_{-0.0018}$ & $^{-0.0032}_{0.0032}$ & $^{0.0015}_{-0.0015}$ & $^{-0.0003}_{0.0003}$ & $^{-0.0029}_{0.0029}$ & $^{0.0018}_{-0.0018}$ & $^{-0.0004}_{0.0004}$ \\ 
weight bTagSF 77 eigenvars Light 7 &  & $^{-0.0023}_{0.0022}$ & $^{-0.0021}_{0.0022}$ & $^{-0.0041}_{0.0041}$ & $^{0.0017}_{-0.0017}$ & $^{0.0018}_{-0.0018}$ & $^{0.0035}_{-0.0034}$ & $^{-0.0027}_{0.0027}$ & $^{-0.0035}_{0.0035}$ & $^{0.0032}_{-0.0032}$ & $^{0.0031}_{-0.0031}$ \\ 
weight bTagSF 77 eigenvars Light 8 &  & $^{-0.0051}_{0.0051}$ & $^{0.0033}_{-0.0032}$ & $^{0.0019}_{-0.0019}$ & $^{0.0019}_{-0.002}$ & $^{-0.0052}_{0.0052}$ & $^{0.002}_{-0.002}$ & $^{-0.0005}_{0.0005}$ & $^{-0.0008}_{0.0008}$ & $^{0.0035}_{-0.0035}$ & $^{-0.0013}_{0.0013}$ \\ 
weight bTagSF 77 eigenvars Light 9 &  & $^{-0.0006}_{0.0006}$ & $^{0.0005}_{-0.0004}$ & $^{-0.0018}_{0.0018}$ & $^{0.0032}_{-0.0032}$ & $^{-0.0018}_{0.0018}$ & $^{-0.0031}_{0.0031}$ & $^{0.0031}_{-0.0031}$ & $^{0.0015}_{-0.0015}$ & $^{0.0005}_{-0.0005}$ & $^{-0.0016}_{0.0016}$ \\ 
weight bTagSF 77 eigenvars Light 10 &  & $^{0.0004}_{-0.0004}$ & $^{0.0011}_{-0.0011}$ & $^{-0.0003}_{0.0003}$ & $^{0.0012}_{-0.0012}$ & $^{-0.0013}_{0.0013}$ & $^{-0.0009}_{0.0009}$ & $^{0.0009}_{-0.0009}$ & $^{0.0004}_{-0.0005}$ & $^{-0.0009}_{0.0009}$ & $^{-0.0002}_{0.0002}$ \\ 
weight bTagSF 77 eigenvars Light 11 &  & $^{0.0}_{0.0} $ & $^{-0.0003}_{0.0003}$ & $^{0.0023}_{-0.0023}$ & $^{-0.001}_{0.0009}$ & $^{0.0016}_{-0.0016}$ & $^{0.0006}_{-0.0007}$ & $^{-0.0014}_{0.0014}$ & $^{-0.0005}_{0.0005}$ & $^{-0.001}_{0.001}$ & $^{0.0}_{0.0} $ \\ 
weight bTagSF 77 eigenvars Light 12 &  & $^{-0.0022}_{0.0022}$ & $^{0.0015}_{-0.0015}$ & $^{0.0}_{0.0} $ & $^{0.0012}_{-0.0012}$ & $^{-0.0016}_{0.0016}$ & $^{-0.0004}_{0.0004}$ & $^{0.0007}_{-0.0007}$ & $^{0.0002}_{-0.0002}$ & $^{0.0}_{0.0} $ & $^{0.0005}_{-0.0005}$ \\ 
weight bTagSF 77 eigenvars Light 13 &  & $^{0.0018}_{-0.0018}$ & $^{0.0011}_{-0.0011}$ & $^{-0.001}_{0.001}$ & $^{-0.0003}_{0.0003}$ & $^{-0.0004}_{0.0004}$ & $^{-0.0002}_{0.0002}$ & $^{0.0002}_{-0.0002}$ & $^{-0.0004}_{0.0004}$ & $^{-0.0003}_{0.0003}$ & $^{-0.0002}_{0.0002}$ \\ 
weight bTagSF 77 eigenvars Light 14 &  & $^{-0.0009}_{0.0009}$ & $^{0.0005}_{-0.0005}$ & $^{0.0}_{0.0} $ & $^{0.0005}_{-0.0005}$ & $^{-0.0002}_{0.0002}$ & $^{-0.0002}_{0.0002}$ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0004}_{-0.0004}$ \\ 
weight bTagSF 77 eigenvars Light 15 &  & $^{-0.0002}_{0.0002}$ & $^{-0.0003}_{0.0003}$ & $^{0.0005}_{-0.0005}$ & $^{0.0001}_{-0.0001}$ & $^{-0.0001}_{0.0001}$ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
weight bTagSF 77 eigenvars Light 16 &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
weight bTagSF 77 extrapolation &  & $^{0.0026}_{-0.0025}$ & $^{-0.0023}_{0.0024}$ & $^{0.002}_{-0.002}$ & $^{-0.0013}_{0.0012}$ & $^{-0.0016}_{0.0016}$ & $^{-0.0012}_{0.0012}$ & $^{-0.0011}_{0.0011}$ & $^{0.0012}_{-0.0011}$ & $^{0.0}_{-0.0001}$ & $^{0.0014}_{-0.0014}$ \\ 
weight bTagSF 77 extrapolation from charmrm &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
weight bTagSF 77 extrapolation from charm &  & $^{0.0001}_{-0.0001}$ & $^{-0.0006}_{0.0006}$ & $^{0.0007}_{-0.0006}$ & $^{-0.0002}_{0.0002}$ & $^{-0.0004}_{0.0004}$ & $^{0.0}_{0.0} $ & $^{-0.0004}_{0.0004}$ & $^{0.0}_{0.0} $ & $^{-0.0003}_{0.0003}$ & $^{0.0011}_{-0.0011}$ \\ 
EG RESOLUTION ALL  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
EG SCALE ALL  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET BJES Response  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 1  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 2  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 3  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 4  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 5  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 6  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 7  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EffectiveNP 8restTerm  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EtaIntercalibration Modelling  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EtaIntercalibration NonClosure  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET EtaIntercalibration TotalStat  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET Flavor Composition  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET Flavor Response  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET Pileup OffsetMu  &  & $^{0.0318}_{-0.0411}$ & $^{0.0011}_{-0.0044}$ & $^{-0.0137}_{-0.0369}$ & $^{0.0363}_{0.012}$ & $^{0.0067}_{0.0055}$ & $^{0.0102}_{-0.0116}$ & $^{-0.0453}_{0.0143}$ & $^{0.0052}_{-0.003}$ & $^{-0.0097}_{0.0096}$ & $^{-0.0114}_{0.0373}$ \\ 
JET 21NP JET Pileup OffsetNPV  &  & $^{-0.0554}_{0.0648}$ & $^{-0.027}_{0.0352}$ & $^{-0.0905}_{-0.0075}$ & $^{0.028}_{0.01}$ & $^{-0.0196}_{0.005}$ & $^{0.0231}_{-0.0485}$ & $^{-0.0207}_{0.005}$ & $^{0.0515}_{-0.0162}$ & $^{0.0463}_{0.0174}$ & $^{0.0268}_{-0.0443}$ \\ 
JET 21NP JET Pileup PtTerm  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET Pileup RhoTopology  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET PunchThrough MC15  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET 21NP JET SingleParticle HighPt  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
JET JER SINGLE NP  &  & $^{0.008}_{0.0} $ & $^{0.0159}_{0.0} $ & $^{0.0911}_{0.0} $ & $^{0.1558}_{0.0} $ & $^{-0.2109}_{0.0} $ & $^{-0.0168}_{0.0} $ & $^{-0.0387}_{0.0} $ & $^{0.0259}_{0.0} $ & $^{0.0235}_{0.0} $ & $^{-0.0331}_{0.0} $ \\ 
MET SoftTrk ResoPara &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MET SoftTrk ResoPerp &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MET SoftTrk Scale &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MUON ID  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MUON MS  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MUON SAGITTA RESBIAS  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MUON SAGITTA RHO  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MUON SCALE  &  & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ & $^{0.0}_{0.0} $ \\ 
MC STAT &  & $^{0.0836}_{0.0} $ & $^{0.0695}_{0.0} $ & $^{0.0488}_{0.0} $ & $^{0.039}_{0.0} $ & $^{0.0203}_{0.0} $ & $^{-0.0067}_{0.0} $ & $^{-0.0284}_{0.0} $ & $^{-0.0401}_{0.0} $ & $^{-0.0568}_{0.0} $ & $^{-0.071}_{0.0} $ \\ 
\midrule 
Total systematics   & +2.3 -2.3 & +1.3 -1.3 & +2.3 -2.3 & +1.6 -1.6 & +0.6 -0.6 & +1.8 -1.8 & +2.0 -2.0 & +1.8 -1.8 & +0.7 -0.8 & +1.5 -1.5\\ 
\midrule 
Data statistics     & $\pm1.1$ & $\pm1.0$ & $\pm1.0$ & $\pm0.9$ & $\pm0.9$ & $\pm0.8$ & $\pm0.8$ & $\pm0.7$ & $\pm0.7$ & $\pm0.7$\\ 
\midrule 
Total uncertainty   & +2.6 -2.6 & +1.7 -1.7 & +2.5 -2.5 & +1.8 -1.8 & +1.1 -1.1 & +2.0 -2.0 & +2.1 -2.1 & +2.0 -2.0 & +1.0 -1.0 & +1.6 -1.6\\ 
\bottomrule 
\end{tabular}

\label{tab:syst_full_dphi_ll_parton_normalised}
\end{table}


==> tables/results_deta_ll_particle.tex <==
\begin{table}[htb]
\caption{Summary of the particle-level absolute and normalised differential cross-sections as a function of $\Delta\eta(\ell^{+},\ell^{-})$, with statistical and systematic uncertainties in each bin.}
\vspace{3mm}
\setlength\extrarowheight{4pt}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\eta(\ell^{+},\ell^{-})$: particle & Cross-section & stat. & syst. & Normalised  & stat. & syst. \\ \relax 
 [unit $\eta$] & [pb/(unit $\eta$)] &  &  & [1/(unit $\eta$)] &  &  \\ 
\midrule
0.0 -- 0.25 & 4.66 & $\pm$ 0.03 & $\pm$ 0.26 & 0.557 & $\pm$ 0.004 & $\pm$ 0.006 \\ 
0.25 -- 0.5 & 4.50 & $\pm$ 0.03 & $\pm$ 0.26 & 0.537 & $\pm$ 0.003 & $\pm$ 0.003 \\ 
0.5 -- 0.75 & 4.34 & $\pm$ 0.03 & $\pm$ 0.27 & 0.518 & $\pm$ 0.003 & $\pm$ 0.004 \\ 
0.75 -- 1.0 & 3.97 & $\pm$ 0.03 & $\pm$ 0.24 & 0.475 & $\pm$ 0.003 & $\pm$ 0.004 \\ 
1.0 -- 1.25 & 3.55 & $\pm$ 0.03 & $\pm$ 0.25 & 0.424 & $\pm$ 0.003 & $\pm$ 0.008 \\ 
1.25 -- 1.5 & 3.05 & $\pm$ 0.03 & $\pm$ 0.17 & 0.364 & $\pm$ 0.003 & $\pm$ 0.004 \\ 
1.5 -- 1.75 & 2.57 & $\pm$ 0.02 & $\pm$ 0.16 & 0.307 & $\pm$ 0.003 & $\pm$ 0.003 \\ 
1.75 -- 2.0 & 2.06 & $\pm$ 0.02 & $\pm$ 0.12 & 0.246 & $\pm$ 0.002 & $\pm$ 0.002 \\ 
2.0 -- 2.5 & 1.35 & $\pm$ 0.01 & $\pm$ 0.08 & 0.162 & $\pm$ 0.001 & $\pm$ 0.002 \\ 
2.5 -- 3.0 & 0.66 & $\pm$ 0.01 & $\pm$ 0.04 & 0.079 & $\pm$ 0.001 & $\pm$ 0.001 \\ 
3.0 -- 3.5 & 0.27 & $\pm$ 0.01 & $\pm$ 0.02 & 0.033 & $\pm$ 0.001 & $\pm$ 0.001 \\ 
3.5 -- 5.0 & 0.038 & $\pm$ 0.001 & $\pm$ 0.003 & 0.0045 & $\pm$ 0.0002 & $\pm$ 0.0003 \\ 
\bottomrule 
\end{tabular}
\label{tab:results_deta_ll_particle}
\end{table}


==> tables/results_dphi.tex <==
\begin{table}
\caption{Summary of the measured absolute differential cross-sections with respect to $\Delta\phi(\ell^{+},\ell^{-})/\pi$ at particle level, along with the relative statistical (Stat.) and systematic (Syst.) uncertainties. The results and uncertainties are rounded according to the recommendations from the Particle Data Group (PDG).}
\centering
\begin{tabular}{c c c c}\toprule 
$X$ & $\frac{\text{d}\sigma_{\ttbar}}{\text{d}X}$ & Stat. & Syst.\\
\midrule 
$\Delta\phi(\ell^{+},\ell^{-})/\pi$: particle & & [\%] & [\%] \\
\midrule 
$0.0$ - $0.1$ &  5.3 $\pm 1.1$ $ +7~-7$\\
$0.1$ - $0.2$ &  5.5 $\pm 1.0$ $ +7~-7$\\
$0.2$ - $0.3$ &  5.9 $\pm 1.0$ $ +7~-7$\\
$0.3$ - $0.4$ &  6.5 $\pm 0.9$ $ +7~-7$\\
$0.4$ - $0.5$ &  7.4 $\pm 0.9$ $ +7~-7$\\
$0.5$ - $0.6$ &  8.4 $\pm 0.8$ $ +7~-7$\\
$0.6$ - $0.7$ &  9.6 $\pm 0.8$ $ +7~-7$\\
$0.7$ - $0.8$ & 10.8 $\pm 0.7$ $ +7~-7$\\
$0.8$ - $0.9$ & 11.9 $\pm 0.7$ $ +7~-7$\\
$0.9$ - $1.0$ & 12.5 $\pm 0.7$ $ +7~-7$\\
\bottomrule 
\end{tabular}
\label{tab:results_v1_dphi_ll_particle}
\end{table}


==> tables/results_dphi_and_deta_parton.tex <==
\begin{table}[htb]
\caption{Summary of the parton-level absolute and normalised differential cross-sections, with statistical and systematic uncertainties in each bin: $|\Delta\phi|$ (top) and $|\Delta\eta|$ (bottom).}
\vspace{3mm}
\setlength\extrarowheight{4pt}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$]: parton & cross section (pb) & stat. & syst. & normalised  & stat. & syst. \\ 
\midrule
0.0 -- 0.1 & 16.91 & 0.18 & $\pm$ 1.03 & 0.863 & 0.009 & $\pm$ 0.007 \\ 
0.1 -- 0.2 & 17.12 & 0.17 & $^{+0.95}_{-0.96}$ & 0.874 & 0.008 & $\pm$ 0.009 \\ 
0.2 -- 0.3 & 17.22 & 0.17 & $^{+1.06}_{-1.08}$ & 0.879 & 0.008 & $^{+0.018}_{-0.019}$ \\ 
0.3 -- 0.4 & 17.95 & 0.17 & $\pm$ 1.1 & 0.917 & 0.008 & $\pm$ 0.008 \\ 
0.4 -- 0.5 & 18.84 & 0.16 & $^{+1.13}_{-1.14}$ & 0.962 & 0.008 & $\pm$ 0.008 \\ 
0.5 -- 0.6 & 19.59 & 0.16 & $^{+1.16}_{-1.18}$ & 1.001 & 0.008 & $\pm$ 0.019 \\ 
0.6 -- 0.7 & 20.43 & 0.16 & $^{+1.13}_{-1.15}$ & 1.043 & 0.008 & $\pm$ 0.012 \\ 
0.7 -- 0.8 & 21.75 & 0.16 & $^{+1.42}_{-1.43}$ & 1.111 & 0.008 & $\pm$ 0.013 \\ 
0.8 -- 0.9 & 22.63 & 0.16 & $^{+1.44}_{-1.45}$ & 1.156 & 0.008 & $\pm$ 0.009 \\ 
0.9 -- 1.0 & 23.37 & 0.16 & $^{+1.44}_{-1.45}$ & 1.194 & 0.008 & $\pm$ 0.013 \\ 
\bottomrule 
\vspace*{1mm}
\end{tabular}
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\eta(\ell^{+},\ell^{-})$: parton & cross section (pb) & stat. & syst. & normalised  & stat. & syst. \\ 
\midrule
0.0 -- 0.25 & 9.04 & 0.06 & $^{+0.47}_{-0.48}$ & 0.463 & 0.003 & $\pm$ 0.011 \\ 
0.25 -- 0.5 & 8.81 & 0.06 & $\pm$ 0.48 & 0.451 & 0.003 & $\pm$ 0.008 \\ 
0.5 -- 0.75 & 8.65 & 0.06 & $^{+0.57}_{-0.58}$ & 0.443 & 0.003 & $\pm$ 0.004 \\ 
0.75 -- 1.0 & 8.1 & 0.06 & $^{+0.45}_{-0.46}$ & 0.415 & 0.003 & $\pm$ 0.007 \\ 
1.0 -- 1.25 & 7.48 & 0.06 & $\pm$ 0.57 & 0.383 & 0.003 & $\pm$ 0.007 \\ 
1.25 -- 1.5 & 6.68 & 0.06 & $\pm$ 0.38 & 0.342 & 0.003 & $\pm$ 0.004 \\ 
1.5 -- 1.75 & 5.94 & 0.06 & $\pm$ 0.33 & 0.304 & 0.003 & $\pm$ 0.004 \\ 
1.75 -- 2.0 & 5.15 & 0.05 & $\pm$ 0.37 & 0.264 & 0.003 & $\pm$ 0.003 \\ 
2.0 -- 2.5 & 3.85 & 0.04 & $\pm$ 0.28 & 0.197 & 0.002 & $\pm$ 0.005 \\ 
2.5 -- 3.0 & 2.42 & 0.03 & $\pm$ 0.20 & 0.124 & 0.002 & $\pm$ 0.005 \\ 
3.0 -- 3.5 & 1.46 & 0.03 & $\pm$ 0.15 & 0.075 & 0.002 & $\pm$ 0.005 \\ 
3.5 -- 5.0 & 0.47 & 0.02 & $\pm$ 0.05 & 0.024 & 0.001 & $\pm$ 0.002 \\ 
\bottomrule 
\end{tabular}
\label{tab:results_dphi_and_deta_parton}
\end{table}


==> tables/results_dphi_ll_particle.tex <==
\begin{table}[htb]
\caption{Summary of the particle-level absolute and normalised differential cross-sections as a function of $\Delta\phi(\ell^{+},\ell^{-})$, with statistical and systematic uncertainties in each bin.}
\vspace{3mm}
\setlength\extrarowheight{4pt}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\phi(\ell^{+},\ell^{-})$: particle & Cross-section & stat. & syst. & Normalised  & stat. & syst. \\ \relax 
 [rad/$\pi$] & [pb/(rad/$\pi$)] &  &  & [1/(rad/$\pi$)] &  &  \\ 
\midrule
0.0 -- 0.1 & 5.59 & $\pm$ 0.06 & $\pm$ 0.35 & 0.667 & $\pm$ 0.007 & $\pm$ 0.012 \\ 
0.1 -- 0.2 & 5.76 & $\pm$ 0.06 & $\pm$ 0.34 & 0.687 & $\pm$ 0.007 & $\pm$ 0.005 \\ 
0.2 -- 0.3 & 6.02 & $\pm$ 0.06 & $\pm$ 0.35 & 0.719 & $\pm$ 0.007 & $\pm$ 0.013 \\ 
0.3 -- 0.4 & 6.68 & $\pm$ 0.06 & $\pm$ 0.39 & 0.797 & $\pm$ 0.007 & $\pm$ 0.008 \\ 
0.4 -- 0.5 & 7.52 & $\pm$ 0.06 & $\pm$ 0.44 & 0.897 & $\pm$ 0.007 & $\pm$ 0.005 \\ 
0.5 -- 0.6 & 8.42 & $\pm$ 0.07 & $\pm$ 0.46 & 1.005 & $\pm$ 0.008 & $\pm$ 0.011 \\ 
0.6 -- 0.7 & 9.47 & $\pm$ 0.07 & $\pm$ 0.56 & 1.130 & $\pm$ 0.008 & $\pm$ 0.006 \\ 
0.7 -- 0.8 & 10.66 & $\pm$ 0.08 & $\pm$ 0.63 & 1.272 & $\pm$ 0.008 & $\pm$ 0.006 \\ 
0.8 -- 0.9 & 11.55 & $\pm$ 0.08 & $\pm$ 0.70 & 1.378 & $\pm$ 0.009 & $\pm$ 0.010 \\ 
0.9 -- 1.0 & 12.12 & $\pm$ 0.08 & $\pm$ 0.73 & 1.447 & $\pm$ 0.009 & $\pm$ 0.013 \\ 
\bottomrule 
\end{tabular}
\label{tab:results_dphi_ll_particle}
\end{table}


==> tables/results_dphi_ll_parton_6bins.tex <==
\begin{table}
\caption{Summary of the parton-level absolute and normalised differential cross-sections in 6 bins as a function of $\Delta\phi(\ell^{+},\ell^{-})$, with statistical and systematic uncertainties in each bin.}
\vspace{3mm}
\setlength\extrarowheight{4pt}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\phi(l^{+},l^{-})$: parton & Cross-section & stat. & syst. & Normalised  & stat. & syst. \\ \relax 
 [rad/$\pi$] & [pb/(rad/$\pi$)] &  &  & [1/(rad/$\pi$)] &  &  \\ 
\midrule
0.00 -- 0.17   & 17.0 & $\pm$ 0.1 & $\pm$ 0.9 & 0.867 & $\pm$ 0.006 & $\pm$ 0.011 \\ 
0.17 -- 0.33   & 17.3 & $\pm$ 0.1 & $\pm$ 1.1 & 0.885 & $\pm$ 0.006 & $\pm$ 0.010 \\ 
0.33 -- 0.50   & 18.5 & $\pm$ 0.1 & $\pm$ 1.1 & 0.946 & $\pm$ 0.006 & $\pm$ 0.007 \\ 
0.50 -- 0.67   & 19.9 & $\pm$ 0.1 & $\pm$ 1.2 & 1.015 & $\pm$ 0.006 & $\pm$ 0.016 \\ 
0.67 -- 0.83   & 21.6 & $\pm$ 0.1 & $\pm$ 1.3 & 1.104 & $\pm$ 0.006 & $\pm$ 0.009 \\ 
0.83 -- 1.00   & 23.2 & $\pm$ 0.1 & $\pm$ 1.5 & 1.184 & $\pm$ 0.006 & $\pm$ 0.013 \\ 
\bottomrule 
\end{tabular}
\label{tab:results_dphi_ll_parton_6bins}
\end{table}


==> tables/results_dphi_ll_parton_normalised.tex <==
\begin{table}
\caption{Summary of the measured normalised differential cross-sections with respect to $\Delta\phi(\ell^{+},\ell^{-})/\pi$ at parton level, along with the relative statistical (Stat.) and systematic (Syst.) uncertainties. The results and uncertainties are rounded according to the recommendations from the Particle Data Group (PDG).}
\centering
\begin{tabular}{c c c c}\toprule 
$X$ & $\frac{1}{\sigma_{\ttbar}}\frac{\text{d}\sigma_{\ttbar}}{\text{d}X}$ & Stat. & Syst.\\
\midrule 
$\Delta\phi(\ell^{+},\ell^{-})/\pi$ & & [\%] & [\%] \\
\midrule 
$0.0$ - $0.1$ & 0.8 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.1$ - $0.2$ & 0.8 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.2$ - $0.3$ & 0.9 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.3$ - $0.4$ & 0.9 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.4$ - $0.5$ & 0.9 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.5$ - $0.6$ & 1.0 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.6$ - $0.7$ & 1.1 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.7$ - $0.8$ & 1.1 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.8$ - $0.9$ & 1.2 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
$0.9$ - $1.0$ & 1.2 & $\pm 0.0$ & $ +0.0$ $-0.0$\\
\bottomrule 
\end{tabular}
\label{tab:results_dphi_ll_parton_normalised}
\end{table}


==> tables/results_dphi_ll_vs_ttbar_m_particle.tex <==
\begin{table}[htb]
\caption{Summary of the particle-level absolute and normalised differential cross-sections as a function of $\Delta\phi(l^{+},l^{-})$ in four regions of $m_{t\bar{t}}$, with statistical and systematic uncertainties in each bin.}
\vspace{3mm}
\setlength\extrarowheight{4pt}
\centering
\begin{tabular}{c c c c c c c c}
\toprule
$\Delta\phi(\ell^{+},\ell^{-})$: particle & Cross-section & stat. & syst. & Normalised  & stat. & syst. \\ \relax 
 [rad/$\pi$] & [pb/(rad/$\pi$)] &  &  & [1/(rad/$\pi$)] &  &  \\ 
\midrule
\multicolumn{7}{l}{$m_{t\bar{t}} < 450$ GeV} \\ 
\midrule
0.0 -- 0.2 & 2.46 & $\pm$ 0.04 & $\pm$ 0.21 & 1.022 & $\pm$ 0.015 & $\pm$ 0.019 \\ 
0.2 -- 0.4 & 2.48 & $\pm$ 0.04 & $\pm$ 0.20 & 1.030 & $\pm$ 0.015 & $\pm$ 0.034 \\ 
0.4 -- 0.6 & 2.46 & $\pm$ 0.04 & $\pm$ 0.20 & 1.023 & $\pm$ 0.015 & $\pm$ 0.023 \\ 
0.6 -- 0.8 & 2.44 & $\pm$ 0.04 & $\pm$ 0.21 & 1.014 & $\pm$ 0.015 & $\pm$ 0.020 \\ 
0.8 -- 1.0 & 2.19 & $\pm$ 0.04 & $\pm$ 0.19 & 0.911 & $\pm$ 0.014 & $\pm$ 0.029 \\ 
\midrule
\multicolumn{7}{l}{$450 \leq m_{t\bar{t}} < 550$ GeV} \\ 
\midrule
0.0 -- 0.3 & 0.84 & $\pm$ 0.02 & $\pm$ 0.08 & 0.569 & $\pm$ 0.011 & $\pm$ 0.033 \\ 
0.3 -- 0.6 & 1.39 & $\pm$ 0.02 & $\pm$ 0.11 & 0.945 & $\pm$ 0.012 & $\pm$ 0.037 \\ 
0.6 -- 0.8 & 1.88 & $\pm$ 0.03 & $\pm$ 0.14 & 1.275 & $\pm$ 0.016 & $\pm$ 0.037 \\ 
0.8 -- 1.0 & 2.15 & $\pm$ 0.03 & $\pm$ 0.16 & 1.454 & $\pm$ 0.017 & $\pm$ 0.057 \\ 
\midrule
\multicolumn{7}{l}{$550 \leq m_{t\bar{t}} < 800$ GeV} \\ 
\midrule
0.0 -- 0.4 & 0.53 & $\pm$ 0.01 & $\pm$ 0.04 & 0.419 & $\pm$ 0.010 & $\pm$ 0.018 \\ 
0.4 -- 0.6 & 1.10 & $\pm$ 0.03 & $\pm$ 0.10 & 0.869 & $\pm$ 0.020 & $\pm$ 0.049 \\ 
0.6 -- 0.8 & 1.81 & $\pm$ 0.03 & $\pm$ 0.15 & 1.426 & $\pm$ 0.022 & $\pm$ 0.065 \\ 
0.8 -- 1.0 & 2.37 & $\pm$ 0.04 & $\pm$ 0.17 & 1.866 & $\pm$ 0.023 & $\pm$ 0.031 \\ 
\midrule
\multicolumn{7}{l}{$m_{t\bar{t}} \geq 800$ GeV} \\ 
\midrule
0.0 -- 0.8 & 0.23 & $\pm$ 0.01 & $\pm$ 0.03 & 0.643 & $\pm$ 0.013 & $\pm$ 0.033 \\ 
0.8 -- 1.0 & 0.87 & $\pm$ 0.02 & $\pm$ 0.10 & 2.427 & $\pm$ 0.052 & $\pm$ 0.126 \\ 
\bottomrule 
\end{tabular}
\label{tab:results_dphi_ll_vs_ttbar_m_particle}
\end{table}


==> tables/results_fsm_systematics.tex <==
\begin{landscape}
\caption{Summary table of the effect of experimental systematic uncertainties on the $f_{SM}$ extraction. Uncertainties which are less than 1\% in all observables are not included in the table (but are included in the $f_{SM}$ significance calculations.)}
\begin{table}
\centering
\begin{tabular}{l c c c c c}
\toprule
Systematic & Inclusive  & $m(t\bar{t}) < 450$ GeV & $450 \leq m(t\bar{t}) < 550$ GeV & $550 \leq m(t\bar{t}) < 800$ GeV & $800 \leq m(t\bar{t})$ GeV \\
\midrule
Radiation systematics (RadHi)                &   0.07 (   5.5 ) &      ( < 1.0 ) & 0.17 (  14.7 ) & 0.51 (  30.2 ) & 0.51 (  22.3 ) \\
Pile-up Effects                              &   0.01 (   1.0 ) &      ( < 1.0 ) &      (   1.0 ) & 0.07 (   3.9 ) & 0.20 (   9.0 ) \\
Matrix Element Generator                     &        ( < 1.0 ) & 0.12 (  10.4 ) & 0.04 (   3.2 ) & 0.05 (   2.7 ) & 0.35 (  15.6 ) \\
Parton Shower and Hadronisation              &        ( < 1.0 ) & 0.03 (   2.5 ) &      ( < 1.0 ) & 0.07 (   4.1 ) & 1.40 (  61.7 ) \\
PDF                                          &        ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) & 0.09 (   3.9 ) \\
Background Modelling                         &        ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) & 0.08 (   3.3 ) \\
Lepton Identification and Reconstruction     &        ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) & 0.07 (   3.0 ) \\
$b$-tagging                                  &        ( < 1.0 ) &      ( < 1.0 ) & 0.02 (   1.9 ) & 0.03 (   1.6 ) & 0.04 (   1.8 ) \\
Jet Identification and Reconstruction        &        ( < 1.0 ) & 0.02 (   1.5 ) & 0.02 (   1.9 ) & 0.11 (   6.3 ) & 0.89 (  39.4 ) \\
Missing Transverse Energy Reconstruction     &        ( < 1.0 ) & 0.02 (   1.7 ) & 0.05 (   3.7 ) & 0.11 (   6.7 ) & 0.86 (  37.8 ) \\
Monte Carlo Statistics                       &        ( < 1.0 ) &      ( < 1.0 ) &      ( < 1.0 ) & 0.03 (   2.0 ) &      ( < 1.0 ) \\
\bottomrule
\end{tabular}
\label{tab:fsm_systematics}
\end{table}

\end{landscape}

==> tables/systematics_deta_ll_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\eta(\ell^{+},\ell^{-})$ at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\tiny
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\eta(\ell^{+},\ell^{-})$ &  0.0 -- 0.25  &  0.25 -- 0.5  &  0.5 -- 0.75  &  0.75 -- 1.0  &  1.0 -- 1.25  &  1.25 -- 1.5  &  1.5 -- 1.75  &  1.75 -- 2.0  &  2.0 -- 2.5  &  2.5 -- 3.0  &  3.0 -- 3.5  &  3.5 -- 5.0 \\ 
\midrule 
Source & \multicolumn{12}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.22$ & $\pm 0.76$ & $\pm 0.02$ & $\pm 0.44$ & $\pm 0.77$ & $\pm 1.06$ & $\pm 1.03$ & $\pm 0.98$ & $\pm 0.53$ & $\pm 0.81$ & $\pm 1.98$ & $\pm 4.55$\\ 
Parton Distribution Function & $\pm 0.58$ & $\pm 0.59$ & $\pm 0.59$ & $\pm 0.58$ & $\pm 0.55$ & $\pm 0.54$ & $\pm 0.56$ & $\pm 0.61$ & $\pm 0.70$ & $\pm 0.92$ & $\pm 1.23$ & $\pm 1.73$\\ 
Parton Shower and Hadronisation & $\pm 3.87$ & $\pm 4.24$ & $\pm 4.94$ & $\pm 4.63$ & $\pm 5.65$ & $\pm 3.91$ & $\pm 4.71$ & $\pm 4.24$ & $\pm 4.15$ & $\pm 4.39$ & $\pm 3.94$ & $\pm 4.48$\\ 
Radiation and Scale Settings & $\pm 0.25$ & $\pm 0.44$ & $\pm 0.56$ & $\pm 0.23$ & $\pm 1.28$ & $\pm 0.18$ & $\pm 0.10$ & $\pm 0.28$ & $\pm 0.86$ & $\pm 1.12$ & $\pm 1.88$ & $\pm 1.42$\\ 
Background Modelling & $\pm 0.91$ & $\pm 0.80$ & $\pm 0.88$ & $\pm 0.81$ & $\pm 0.92$ & $\pm 0.83$ & $\pm 1.05$ & $\pm 1.37$ & $\pm 1.26$ & $\pm 1.28$ & $\pm 2.05$ & $\pm 2.83$\\ 
Pile-up Effects & $\pm 1.32$ & $\pm 1.38$ & $\pm 1.18$ & $\pm 1.24$ & $\pm 1.20$ & $\pm 1.28$ & $\pm 1.02$ & $\pm 1.42$ & $\pm 0.82$ & $\pm 1.58$ & $\pm 0.79$ & $\pm 2.19$\\ 
Luminosity & $\pm 2.27$ & $\pm 2.27$ & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.25$ & $\pm 2.25$ & $\pm 2.24$ & $\pm 2.24$ & $\pm 2.25$ & $\pm 2.26$ & $\pm 2.28$\\ 
Lepton Identification and Reconstruction & $\pm 1.20$ & $\pm 1.21$ & $\pm 1.21$ & $\pm 1.21$ & $\pm 1.22$ & $\pm 1.20$ & $\pm 1.22$ & $\pm 1.23$ & $\pm 1.27$ & $\pm 1.29$ & $\pm 1.40$ & $\pm 1.58$\\ 
Jet Identification and Reconstruction & $\pm 1.91$ & $\pm 1.80$ & $\pm 1.86$ & $\pm 1.79$ & $\pm 1.88$ & $\pm 1.75$ & $\pm 1.80$ & $\pm 1.84$ & $\pm 1.86$ & $\pm 1.69$ & $\pm 2.08$ & $\pm 1.59$\\ 
$b$-tagging & $\pm 1.33$ & $\pm 1.34$ & $\pm 1.29$ & $\pm 1.31$ & $\pm 1.35$ & $\pm 1.33$ & $\pm 1.32$ & $\pm 1.30$ & $\pm 1.32$ & $\pm 1.31$ & $\pm 1.33$ & $\pm 1.37$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.26$ & $\pm 0.26$ & $\pm 0.26$ & $\pm 0.28$ & $\pm 0.29$ & $\pm 0.31$ & $\pm 0.34$ & $\pm 0.38$ & $\pm 0.34$ & $\pm 0.49$ & $\pm 0.79$ & $\pm 1.25$\\ 
\midrule 
Total systematics   & $\pm5.61$ & $\pm5.78$ & $\pm6.25$ & $\pm5.98$ & $\pm6.98$ & $\pm5.52$ & $\pm6.11$ & $\pm5.92$ & $\pm5.74$ & $\pm6.14$ & $\pm6.57$ & $\pm8.76$\\ 
\midrule 
Data statistics     & $\pm0.70$ & $\pm0.70$ & $\pm0.71$ & $\pm0.74$ & $\pm0.78$ & $\pm0.84$ & $\pm0.93$ & $\pm1.04$ & $\pm0.92$ & $\pm1.33$ & $\pm2.10$ & $\pm3.42$\\ 
\midrule 
Total uncertainty   & $\pm5.65$ & $\pm5.82$ & $\pm6.29$ & $\pm6.03$ & $\pm7.02$ & $\pm5.59$ & $\pm6.18$ & $\pm6.01$ & $\pm5.81$ & $\pm6.28$ & $\pm6.89$ & $\pm9.40$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_deta_ll_particle_absolute}
\end{table}


==> tables/systematics_deta_ll_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\eta(\ell^{+},\ell^{-})$ at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\tiny
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\eta(\ell^{+},\ell^{-})$ &  0.0 -- 0.25  &  0.25 -- 0.5  &  0.5 -- 0.75  &  0.75 -- 1.0  &  1.0 -- 1.25  &  1.25 -- 1.5  &  1.5 -- 1.75  &  1.75 -- 2.0  &  2.0 -- 2.5  &  2.5 -- 3.0  &  3.0 -- 3.5  &  3.5 -- 5.0 \\ 
\midrule 
Source & \multicolumn{12}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.80$ & $\pm 0.36$ & $\pm 0.41$ & $\pm 0.05$ & $\pm 1.14$ & $\pm 0.65$ & $\pm 0.62$ & $\pm 0.56$ & $\pm 0.92$ & $\pm 1.19$ & $\pm 2.35$ & $\pm 4.46$\\ 
Parton Distribution Function & $\pm 0.21$ & $\pm 0.20$ & $\pm 0.16$ & $\pm 0.11$ & $\pm 0.02$ & $\pm 0.08$ & $\pm 0.20$ & $\pm 0.32$ & $\pm 0.54$ & $\pm 0.88$ & $\pm 1.27$ & $\pm 1.85$\\ 
Parton Shower and Hadronisation & $\pm 0.55$ & $\pm 0.21$ & $\pm 0.44$ & $\pm 0.18$ & $\pm 1.12$ & $\pm 0.55$ & $\pm 0.25$ & $\pm 0.29$ & $\pm 0.34$ & $\pm 0.13$ & $\pm 0.60$ & $\pm 0.15$\\ 
Radiation and Scale Settings & $\pm 0.19$ & $ 0.0 $ & $\pm 0.13$ & $\pm 0.66$ & $\pm 0.84$ & $\pm 0.61$ & $\pm 0.33$ & $\pm 0.16$ & $\pm 0.43$ & $\pm 0.70$ & $\pm 1.46$ & $\pm 1.01$\\ 
Background Modelling & $\pm 0.12$ & $\pm 0.19$ & $\pm 0.32$ & $\pm 0.16$ & $\pm 0.13$ & $\pm 0.15$ & $\pm 0.16$ & $\pm 0.50$ & $\pm 0.47$ & $\pm 0.38$ & $\pm 1.43$ & $\pm 2.50$\\ 
Pile-up Effects & $\pm 0.08$ & $\pm 0.19$ & $\pm 0.05$ & $\pm 0.07$ & $\pm 0.03$ & $\pm 0.10$ & $\pm 0.22$ & $\pm 0.18$ & $\pm 0.42$ & $\pm 0.35$ & $\pm 0.53$ & $\pm 0.97$\\ 
Luminosity & $\pm 0.02$ & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $\pm 0.01$ & $\pm 0.01$ & $\pm 0.01$ & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $\pm 0.02$\\ 
Lepton Identification and Reconstruction & $\pm 0.05$ & $\pm 0.03$ & $\pm 0.04$ & $\pm 0.10$ & $\pm 0.04$ & $\pm 0.05$ & $\pm 0.04$ & $\pm 0.06$ & $\pm 0.12$ & $\pm 0.16$ & $\pm 0.38$ & $\pm 0.53$\\ 
Jet Identification and Reconstruction & $\pm 0.17$ & $\pm 0.12$ & $\pm 0.08$ & $\pm 0.07$ & $\pm 0.13$ & $\pm 0.16$ & $\pm 0.07$ & $\pm 0.15$ & $\pm 0.09$ & $\pm 0.36$ & $\pm 0.35$ & $\pm 1.40$\\ 
$b$-tagging & $\pm 0.04$ & $\pm 0.03$ & $\pm 0.04$ & $\pm 0.05$ & $\pm 0.04$ & $\pm 0.06$ & $\pm 0.03$ & $\pm 0.04$ & $\pm 0.02$ & $\pm 0.04$ & $\pm 0.09$ & $\pm 0.07$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.24$ & $\pm 0.24$ & $\pm 0.25$ & $\pm 0.26$ & $\pm 0.27$ & $\pm 0.30$ & $\pm 0.33$ & $\pm 0.36$ & $\pm 0.32$ & $\pm 0.48$ & $\pm 0.78$ & $\pm 1.25$\\ 
\midrule 
Total systematics   & $\pm1.07$ & $\pm0.60$ & $\pm0.76$ & $\pm0.77$ & $\pm1.84$ & $\pm1.12$ & $\pm0.88$ & $\pm0.99$ & $\pm1.40$ & $\pm1.83$ & $\pm3.58$ & $\pm5.95$\\ 
\midrule 
Data statistics     & $\pm0.65$ & $\pm0.65$ & $\pm0.66$ & $\pm0.70$ & $\pm0.74$ & $\pm0.80$ & $\pm0.89$ & $\pm1.01$ & $\pm0.88$ & $\pm1.30$ & $\pm2.08$ & $\pm3.40$\\ 
\midrule 
Total uncertainty   & $\pm1.25$ & $\pm0.88$ & $\pm1.01$ & $\pm1.04$ & $\pm1.98$ & $\pm1.38$ & $\pm1.26$ & $\pm1.41$ & $\pm1.66$ & $\pm2.24$ & $\pm4.14$ & $\pm6.85$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_deta_ll_particle_normalised}
\end{table}


==> tables/systematics_deta_ll_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\eta(\ell^{+},\ell^{-})$ at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\tiny
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\eta(\ell^{+},\ell^{-})$ &  0.0 -- 0.25  &  0.25 -- 0.5  &  0.5 -- 0.75  &  0.75 -- 1.0  &  1.0 -- 1.25  &  1.25 -- 1.5  &  1.5 -- 1.75  &  1.75 -- 2.0  &  2.0 -- 2.5  &  2.5 -- 3.0  &  3.0 -- 3.5  &  3.5 -- 5.0 \\ 
\midrule 
Source & \multicolumn{12}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.12$ & $\pm 0.79$ & $\pm 0.18$ & $\pm 0.80$ & $\pm 0.94$ & $\pm 0.05$ & $\pm 0.07$ & $\pm 1.28$ & $\pm 2.96$ & $\pm 4.15$ & $\pm 6.92$ & $\pm 3.67$\\ 
Parton Distribution Function & $\pm 0.58$ & $\pm 0.59$ & $\pm 0.60$ & $\pm 0.58$ & $\pm 0.55$ & $\pm 0.54$ & $\pm 0.56$ & $\pm 0.61$ & $\pm 0.70$ & $\pm 0.92$ & $\pm 1.23$ & $\pm 1.73$\\ 
Parton Shower and Hadronisation & $\pm 3.46$ & $\pm 3.88$ & $\pm 5.53$ & $\pm 4.14$ & $\pm 6.38$ & $\pm 4.32$ & $\pm 4.17$ & $\pm 5.81$ & $\pm 5.36$ & $\pm 5.94$ & $\pm 5.93$ & $\pm 9.57$\\ 
Radiation and Scale Settings & $\pm 0.23$ & $\pm 0.01$ & $\pm 0.38$ & $\pm 0.44$ & $\pm 1.31$ & $\pm 0.13$ & $\pm 0.29$ & $\pm 0.41$ & $\pm 0.23$ & $\pm 0.91$ & $\pm 0.59$ & $\pm 3.02$\\ 
Background Modelling & $\pm 0.91$ & $\pm 0.80$ & $\pm 0.88$ & $\pm 0.81$ & $\pm 0.92$ & $\pm 0.83$ & $\pm 1.05$ & $\pm 1.38$ & $\pm 1.26$ & $\pm 1.28$ & $\pm 2.05$ & $\pm 2.84$\\ 
Pile-up Effects & $\pm 1.32$ & $\pm 1.38$ & $\pm 1.18$ & $\pm 1.24$ & $\pm 1.20$ & $\pm 1.28$ & $\pm 1.02$ & $\pm 1.42$ & $\pm 0.82$ & $\pm 1.58$ & $\pm 0.79$ & $\pm 2.19$\\ 
Luminosity & $\pm 2.27$ & $\pm 2.27$ & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.25$ & $\pm 2.25$ & $\pm 2.24$ & $\pm 2.24$ & $\pm 2.25$ & $\pm 2.26$ & $\pm 2.28$\\ 
Lepton Identification and Reconstruction & $\pm 1.20$ & $\pm 1.21$ & $\pm 1.21$ & $\pm 1.21$ & $\pm 1.22$ & $\pm 1.20$ & $\pm 1.22$ & $\pm 1.23$ & $\pm 1.27$ & $\pm 1.29$ & $\pm 1.40$ & $\pm 1.58$\\ 
Jet Identification and Reconstruction & $\pm 1.91$ & $\pm 1.80$ & $\pm 1.86$ & $\pm 1.79$ & $\pm 1.88$ & $\pm 1.75$ & $\pm 1.80$ & $\pm 1.84$ & $\pm 1.86$ & $\pm 1.69$ & $\pm 2.08$ & $\pm 1.59$\\ 
$b$-tagging & $\pm 1.33$ & $\pm 1.34$ & $\pm 1.29$ & $\pm 1.31$ & $\pm 1.35$ & $\pm 1.33$ & $\pm 1.32$ & $\pm 1.30$ & $\pm 1.32$ & $\pm 1.31$ & $\pm 1.33$ & $\pm 1.37$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.26$ & $\pm 0.26$ & $\pm 0.27$ & $\pm 0.28$ & $\pm 0.30$ & $\pm 0.31$ & $\pm 0.34$ & $\pm 0.39$ & $\pm 0.34$ & $\pm 0.50$ & $\pm 0.81$ & $\pm 1.28$\\ 
\midrule 
Total systematics   & $\pm5.32$ & $\pm5.50$ & $\pm6.72$ & $\pm5.66$ & $\pm7.61$ & $\pm5.72$ & $\pm5.62$ & $\pm7.19$ & $\pm7.23$ & $\pm8.36$ & $\pm10.18$ & $\pm12.18$\\ 
\midrule 
Data statistics     & $\pm0.71$ & $\pm0.71$ & $\pm0.72$ & $\pm0.76$ & $\pm0.80$ & $\pm0.86$ & $\pm0.94$ & $\pm1.06$ & $\pm0.93$ & $\pm1.34$ & $\pm2.11$ & $\pm3.39$\\ 
\midrule 
Total uncertainty   & $\pm5.36$ & $\pm5.55$ & $\pm6.75$ & $\pm5.71$ & $\pm7.65$ & $\pm5.78$ & $\pm5.70$ & $\pm7.26$ & $\pm7.29$ & $\pm8.47$ & $\pm10.39$ & $\pm12.64$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_deta_ll_parton_absolute}
\end{table}


==> tables/systematics_deta_ll_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\eta(\ell^{+},\ell^{-})$ at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\tiny
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\eta(\ell^{+},\ell^{-})$ &  0.0 -- 0.25  &  0.25 -- 0.5  &  0.5 -- 0.75  &  0.75 -- 1.0  &  1.0 -- 1.25  &  1.25 -- 1.5  &  1.5 -- 1.75  &  1.75 -- 2.0  &  2.0 -- 2.5  &  2.5 -- 3.0  &  3.0 -- 3.5  &  3.5 -- 5.0 \\ 
\midrule 
Source & \multicolumn{12}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.76$ & $\pm 1.43$ & $\pm 0.48$ & $\pm 1.44$ & $\pm 0.27$ & $\pm 0.70$ & $\pm 0.72$ & $\pm 0.60$ & $\pm 2.24$ & $\pm 3.41$ & $\pm 6.12$ & $\pm 3.60$\\ 
Parton Distribution Function & $\pm 0.26$ & $\pm 0.25$ & $\pm 0.21$ & $\pm 0.16$ & $\pm 0.08$ & $\pm 0.03$ & $\pm 0.14$ & $\pm 0.27$ & $\pm 0.48$ & $\pm 0.82$ & $\pm 1.21$ & $\pm 1.80$\\ 
Parton Shower and Hadronisation & $\pm 1.46$ & $\pm 1.08$ & $\pm 0.52$ & $\pm 0.83$ & $\pm 1.33$ & $\pm 0.65$ & $\pm 0.79$ & $\pm 0.76$ & $\pm 0.36$ & $\pm 0.90$ & $\pm 0.87$ & $\pm 4.41$\\ 
Radiation and Scale Settings & $\pm 0.24$ & $ 0.0 $ & $\pm 0.39$ & $\pm 0.43$ & $\pm 1.32$ & $\pm 0.12$ & $\pm 0.28$ & $\pm 0.42$ & $\pm 0.24$ & $\pm 0.90$ & $\pm 0.58$ & $\pm 3.01$\\ 
Background Modelling & $\pm 0.12$ & $\pm 0.25$ & $\pm 0.42$ & $\pm 0.26$ & $\pm 0.24$ & $\pm 0.25$ & $\pm 0.14$ & $\pm 0.52$ & $\pm 0.37$ & $\pm 0.38$ & $\pm 1.32$ & $\pm 2.40$\\ 
Pile-up Effects & $\pm 0.07$ & $\pm 0.18$ & $\pm 0.07$ & $\pm 0.08$ & $\pm 0.05$ & $\pm 0.09$ & $\pm 0.24$ & $\pm 0.17$ & $\pm 0.44$ & $\pm 0.34$ & $\pm 0.54$ & $\pm 0.95$\\ 
Luminosity & $\pm 0.02$ & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $\pm 0.01$ & $\pm 0.01$ & $\pm 0.01$ & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $\pm 0.02$\\ 
Lepton Identification and Reconstruction & $\pm 0.08$ & $\pm 0.06$ & $\pm 0.06$ & $\pm 0.11$ & $\pm 0.06$ & $\pm 0.06$ & $\pm 0.05$ & $\pm 0.05$ & $\pm 0.10$ & $\pm 0.15$ & $\pm 0.36$ & $\pm 0.50$\\ 
Jet Identification and Reconstruction & $\pm 0.21$ & $\pm 0.10$ & $\pm 0.12$ & $\pm 0.07$ & $\pm 0.15$ & $\pm 0.15$ & $\pm 0.08$ & $\pm 0.16$ & $\pm 0.11$ & $\pm 0.32$ & $\pm 0.36$ & $\pm 1.36$\\ 
$b$-tagging & $\pm 0.04$ & $\pm 0.04$ & $\pm 0.04$ & $\pm 0.05$ & $\pm 0.04$ & $\pm 0.06$ & $\pm 0.03$ & $\pm 0.04$ & $\pm 0.02$ & $\pm 0.03$ & $\pm 0.09$ & $\pm 0.07$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.25$ & $\pm 0.25$ & $\pm 0.26$ & $\pm 0.27$ & $\pm 0.29$ & $\pm 0.31$ & $\pm 0.33$ & $\pm 0.38$ & $\pm 0.33$ & $\pm 0.48$ & $\pm 0.79$ & $\pm 1.26$\\ 
\midrule 
Total systematics   & $\pm2.35$ & $\pm1.86$ & $\pm0.98$ & $\pm1.77$ & $\pm1.94$ & $\pm1.06$ & $\pm1.20$ & $\pm1.29$ & $\pm2.43$ & $\pm3.81$ & $\pm6.56$ & $\pm7.42$\\ 
\midrule 
Data statistics     & $\pm0.69$ & $\pm0.69$ & $\pm0.70$ & $\pm0.73$ & $\pm0.77$ & $\pm0.83$ & $\pm0.92$ & $\pm1.03$ & $\pm0.88$ & $\pm1.29$ & $\pm2.05$ & $\pm3.28$\\ 
\midrule 
Total uncertainty   & $\pm2.44$ & $\pm1.98$ & $\pm1.21$ & $\pm1.92$ & $\pm2.09$ & $\pm1.35$ & $\pm1.51$ & $\pm1.65$ & $\pm2.59$ & $\pm4.02$ & $\pm6.87$ & $\pm8.11$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_deta_ll_parton_normalised}
\end{table}


==> tables/systematics_dphi_ll_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.1  &  0.1 -- 0.2  &  0.2 -- 0.3  &  0.3 -- 0.4  &  0.4 -- 0.5  &  0.5 -- 0.6  &  0.6 -- 0.7  &  0.7 -- 0.8  &  0.8 -- 0.9  &  0.9 -- 1.0 \\ 
\midrule 
Source & \multicolumn{10}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.07$ & $\pm 0.25$ & $\pm 1.78$ & $\pm 0.37$ & $\pm 0.22$ & $\pm 0.34$ & $\pm 0.53$ & $\pm 0.61$ & $\pm 0.94$ & $\pm 0.69$\\ 
Parton Distribution Function & $\pm 0.77$ & $\pm 0.78$ & $\pm 0.76$ & $\pm 0.72$ & $\pm 0.65$ & $\pm 0.59$ & $\pm 0.52$ & $\pm 0.47$ & $\pm 0.42$ & $\pm 0.39$\\ 
Parton Shower and Hadronisation & $\pm 4.96$ & $\pm 4.43$ & $\pm 4.14$ & $\pm 4.40$ & $\pm 4.45$ & $\pm 3.92$ & $\pm 4.59$ & $\pm 4.48$ & $\pm 4.54$ & $\pm 4.51$\\ 
Radiation and Scale Settings & $\pm 0.87$ & $\pm 0.71$ & $\pm 0.53$ & $\pm 0.31$ & $\pm 0.08$ & $\pm 0.07$ & $\pm 0.73$ & $\pm 0.58$ & $\pm 0.14$ & $\pm 1.02$\\ 
Background Modelling & $\pm 0.85$ & $\pm 0.76$ & $\pm 0.94$ & $\pm 1.00$ & $\pm 0.98$ & $\pm 0.97$ & $\pm 0.84$ & $\pm 0.97$ & $\pm 1.04$ & $\pm 1.05$\\ 
Pile-up Effects & $\pm 0.94$ & $\pm 1.55$ & $\pm 1.54$ & $\pm 1.36$ & $\pm 1.28$ & $\pm 1.52$ & $\pm 1.12$ & $\pm 1.15$ & $\pm 1.25$ & $\pm 0.96$\\ 
Luminosity & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.25$ & $\pm 2.25$ & $\pm 2.26$ & $\pm 2.25$\\ 
Lepton Identification and Reconstruction & $\pm 1.18$ & $\pm 1.18$ & $\pm 1.17$ & $\pm 1.17$ & $\pm 1.17$ & $\pm 1.18$ & $\pm 1.20$ & $\pm 1.23$ & $\pm 1.29$ & $\pm 1.32$\\ 
Jet Identification and Reconstruction & $\pm 1.56$ & $\pm 1.63$ & $\pm 1.64$ & $\pm 1.55$ & $\pm 1.83$ & $\pm 1.89$ & $\pm 1.90$ & $\pm 1.92$ & $\pm 1.89$ & $\pm 2.00$\\ 
$b$-tagging & $\pm 1.31$ & $\pm 1.30$ & $\pm 1.30$ & $\pm 1.33$ & $\pm 1.32$ & $\pm 1.30$ & $\pm 1.31$ & $\pm 1.32$ & $\pm 1.34$ & $\pm 1.35$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.39$ & $\pm 0.38$ & $\pm 0.36$ & $\pm 0.34$ & $\pm 0.32$ & $\pm 0.30$ & $\pm 0.28$ & $\pm 0.26$ & $\pm 0.25$ & $\pm 0.24$\\ 
\midrule 
Total systematics   & $\pm6.29$ & $\pm5.90$ & $\pm5.95$ & $\pm5.81$ & $\pm5.88$ & $\pm5.56$ & $\pm6.00$ & $\pm5.95$ & $\pm6.05$ & $\pm6.06$\\ 
\midrule 
Data statistics     & $\pm1.05$ & $\pm0.99$ & $\pm0.97$ & $\pm0.92$ & $\pm0.86$ & $\pm0.81$ & $\pm0.76$ & $\pm0.71$ & $\pm0.68$ & $\pm0.66$\\ 
\midrule 
Total uncertainty   & $\pm6.38$ & $\pm5.98$ & $\pm6.03$ & $\pm5.88$ & $\pm5.94$ & $\pm5.62$ & $\pm6.05$ & $\pm5.99$ & $\pm6.08$ & $\pm6.09$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_particle_absolute}
\end{table}


==> tables/systematics_dphi_ll_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.1  &  0.1 -- 0.2  &  0.2 -- 0.3  &  0.3 -- 0.4  &  0.4 -- 0.5  &  0.5 -- 0.6  &  0.6 -- 0.7  &  0.7 -- 0.8  &  0.8 -- 0.9  &  0.9 -- 1.0 \\ 
\midrule 
Source & \multicolumn{10}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.44$ & $\pm 0.15$ & $\pm 1.35$ & $\pm 0.76$ & $\pm 0.18$ & $\pm 0.74$ & $\pm 0.12$ & $\pm 0.21$ & $\pm 0.52$ & $\pm 0.28$\\ 
Parton Distribution Function & $\pm 0.32$ & $\pm 0.33$ & $\pm 0.30$ & $\pm 0.25$ & $\pm 0.16$ & $\pm 0.08$ & $\pm 0.03$ & $\pm 0.14$ & $\pm 0.24$ & $\pm 0.32$\\ 
Parton Shower and Hadronisation & $\pm 0.57$ & $\pm 0.05$ & $\pm 0.28$ & $ 0.0 $ & $\pm 0.02$ & $\pm 0.48$ & $\pm 0.15$ & $ 0.0 $ & $\pm 0.06$ & $ 0.0 $\\ 
Radiation and Scale Settings & $\pm 0.45$ & $\pm 0.30$ & $\pm 0.95$ & $\pm 0.11$ & $\pm 0.34$ & $\pm 0.49$ & $\pm 0.30$ & $\pm 0.16$ & $\pm 0.28$ & $\pm 0.60$\\ 
Background Modelling & $\pm 0.17$ & $\pm 0.22$ & $\pm 0.17$ & $\pm 0.40$ & $\pm 0.18$ & $\pm 0.13$ & $\pm 0.12$ & $\pm 0.18$ & $\pm 0.11$ & $\pm 0.13$\\ 
Pile-up Effects & $\pm 0.30$ & $\pm 0.32$ & $\pm 0.35$ & $\pm 0.14$ & $\pm 0.06$ & $\pm 0.29$ & $\pm 0.12$ & $\pm 0.09$ & $\pm 0.07$ & $\pm 0.28$\\ 
Luminosity & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.10$ & $\pm 0.13$ & $\pm 0.11$ & $\pm 0.09$ & $\pm 0.08$ & $\pm 0.07$ & $\pm 0.03$ & $\pm 0.06$ & $\pm 0.12$ & $\pm 0.14$\\ 
Jet Identification and Reconstruction & $\pm 0.30$ & $\pm 0.30$ & $\pm 0.48$ & $\pm 0.27$ & $\pm 0.25$ & $\pm 0.11$ & $\pm 0.12$ & $\pm 0.16$ & $\pm 0.15$ & $\pm 0.21$\\ 
$b$-tagging & $\pm 0.07$ & $\pm 0.05$ & $\pm 0.06$ & $\pm 0.04$ & $\pm 0.03$ & $\pm 0.03$ & $\pm 0.02$ & $\pm 0.03$ & $\pm 0.04$ & $\pm 0.05$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.38$ & $\pm 0.36$ & $\pm 0.34$ & $\pm 0.33$ & $\pm 0.31$ & $\pm 0.28$ & $\pm 0.26$ & $\pm 0.25$ & $\pm 0.23$ & $\pm 0.22$\\ 
\midrule 
Total systematics   & $\pm1.75$ & $\pm0.78$ & $\pm1.85$ & $\pm1.02$ & $\pm0.61$ & $\pm1.10$ & $\pm0.49$ & $\pm0.47$ & $\pm0.73$ & $\pm0.87$\\ 
\midrule 
Data statistics     & $\pm1.01$ & $\pm0.95$ & $\pm0.93$ & $\pm0.88$ & $\pm0.82$ & $\pm0.77$ & $\pm0.72$ & $\pm0.67$ & $\pm0.64$ & $\pm0.62$\\ 
\midrule 
Total uncertainty   & $\pm2.03$ & $\pm1.23$ & $\pm2.07$ & $\pm1.35$ & $\pm1.02$ & $\pm1.34$ & $\pm0.87$ & $\pm0.82$ & $\pm0.97$ & $\pm1.07$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_particle_normalised}
\end{table}


==> tables/systematics_dphi_ll_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.1  &  0.1 -- 0.2  &  0.2 -- 0.3  &  0.3 -- 0.4  &  0.4 -- 0.5  &  0.5 -- 0.6  &  0.6 -- 0.7  &  0.7 -- 0.8  &  0.8 -- 0.9  &  0.9 -- 1.0 \\ 
\midrule 
Source & \multicolumn{10}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.57$ & $\pm 0.11$ & $\pm 1.23$ & $\pm 0.95$ & $\pm 0.06$ & $\pm 2.19$ & $\pm 1.14$ & $\pm 0.10$ & $\pm 0.73$ & $\pm 0.04$\\ 
Parton Distribution Function & $\pm 0.77$ & $\pm 0.78$ & $\pm 0.76$ & $\pm 0.72$ & $\pm 0.65$ & $\pm 0.59$ & $\pm 0.52$ & $\pm 0.47$ & $\pm 0.42$ & $\pm 0.39$\\ 
Parton Shower and Hadronisation & $\pm 4.84$ & $\pm 4.11$ & $\pm 4.71$ & $\pm 4.76$ & $\pm 4.66$ & $\pm 4.00$ & $\pm 3.98$ & $\pm 5.26$ & $\pm 4.99$ & $\pm 4.77$\\ 
Radiation and Scale Settings & $\pm 0.35$ & $\pm 0.50$ & $\pm 0.94$ & $\pm 0.26$ & $\pm 0.51$ & $\pm 0.31$ & $\pm 0.68$ & $\pm 0.94$ & $\pm 0.63$ & $\pm 0.87$\\ 
Background Modelling & $\pm 0.85$ & $\pm 0.76$ & $\pm 0.94$ & $\pm 1.00$ & $\pm 0.98$ & $\pm 0.97$ & $\pm 0.84$ & $\pm 0.97$ & $\pm 1.04$ & $\pm 1.05$\\ 
Pile-up Effects & $\pm 0.94$ & $\pm 1.55$ & $\pm 1.54$ & $\pm 1.36$ & $\pm 1.28$ & $\pm 1.52$ & $\pm 1.11$ & $\pm 1.15$ & $\pm 1.25$ & $\pm 0.96$\\ 
Luminosity & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.25$ & $\pm 2.25$ & $\pm 2.26$ & $\pm 2.25$\\ 
Lepton Identification and Reconstruction & $\pm 1.18$ & $\pm 1.18$ & $\pm 1.17$ & $\pm 1.17$ & $\pm 1.17$ & $\pm 1.18$ & $\pm 1.20$ & $\pm 1.23$ & $\pm 1.29$ & $\pm 1.32$\\ 
Jet Identification and Reconstruction & $\pm 1.56$ & $\pm 1.63$ & $\pm 1.64$ & $\pm 1.55$ & $\pm 1.83$ & $\pm 1.89$ & $\pm 1.90$ & $\pm 1.92$ & $\pm 1.89$ & $\pm 2.00$\\ 
$b$-tagging & $\pm 1.31$ & $\pm 1.30$ & $\pm 1.30$ & $\pm 1.33$ & $\pm 1.32$ & $\pm 1.30$ & $\pm 1.31$ & $\pm 1.32$ & $\pm 1.34$ & $\pm 1.35$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.39$ & $\pm 0.38$ & $\pm 0.36$ & $\pm 0.34$ & $\pm 0.32$ & $\pm 0.30$ & $\pm 0.28$ & $\pm 0.26$ & $\pm 0.25$ & $\pm 0.24$\\ 
\midrule 
Total systematics   & $\pm6.07$ & $\pm5.64$ & $\pm6.28$ & $\pm6.14$ & $\pm6.06$ & $\pm6.02$ & $\pm5.63$ & $\pm6.57$ & $\pm6.39$ & $\pm6.20$\\ 
\midrule 
Data statistics     & $\pm1.06$ & $\pm1.00$ & $\pm0.98$ & $\pm0.93$ & $\pm0.87$ & $\pm0.83$ & $\pm0.78$ & $\pm0.73$ & $\pm0.70$ & $\pm0.68$\\ 
\midrule 
Total uncertainty   & $\pm6.16$ & $\pm5.72$ & $\pm6.36$ & $\pm6.21$ & $\pm6.12$ & $\pm6.08$ & $\pm5.69$ & $\pm6.61$ & $\pm6.43$ & $\pm6.23$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_parton_absolute}
\end{table}


==> tables/systematics_dphi_ll_parton_absolute_6bins.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] in 6 bins at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.17  &  0.17 -- 0.33  &  0.33 -- 0.50  &  0.50 -- 0.67  &  0.67 -- 0.83  &  0.83 -- 1.0 \\ 
\midrule 
Source & \multicolumn{6}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.36$ & $\pm 0.56$ & $\pm 0.0 $ & $\pm 1.91$ & $\pm 0.52$ & $\pm 0.08$\\ 
Parton Distribution Function & $\pm 0.78$ & $\pm 0.76$ & $\pm 0.68$ & $\pm 0.57$ & $\pm 0.46$ & $\pm 0.40$\\ 
Parton Shower and Hadronisation & $\pm 4.14$ & $\pm 5.15$ & $\pm 4.53$ & $\pm 3.97$ & $\pm 4.77$ & $\pm 5.05$\\ 
Radiation and Scale Settings & $\pm 0.59$ & $\pm 0.61$ & $\pm 0.39$ & $\pm 0.06$ & $\pm 0.80$ & $\pm 0.93$\\ 
Background Modelling & $\pm 0.95$ & $\pm 0.95$ & $\pm 1.12$ & $\pm 1.01$ & $\pm 1.11$ & $\pm 1.3$\\ 
Pileup Effects & $\pm 1.14$ & $\pm 1.59$ & $\pm 1.28$ & $\pm 1.36$ & $\pm 1.15$ & $\pm 1.07$\\ 
Luminosity & $\pm 2.27$ & $\pm 2.27$ & $\pm 2.26$ & $\pm 2.26$ & $\pm 2.25$ & $\pm 2.25$\\ 
Lepton Identification and Reconstruction & $\pm 1.18$ & $\pm 1.17$ & $\pm 1.17$ & $\pm 1.18$ & $\pm 1.23$ & $\pm 1.31$\\ 
Jet Identification and Reconstruction & $\pm 1.56$ & $\pm 1.58$ & $\pm 1.77$ & $\pm 1.84$ & $\pm 1.97$ & $\pm 1.94$\\ 
$b$-tagging & $\pm 1.30$ & $\pm 1.29$ & $\pm 1.33$ & $\pm 1.31$ & $\pm 1.32$ & $\pm 1.35$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.30$ & $\pm 0.29$ & $\pm 0.25$ & $\pm 0.23$ & $\pm 0.20$ & $\pm 0.19$\\ 
\midrule 
Total systematics   & $\pm5.58$ & $\pm6.48$ & $\pm5.96$ & $\pm5.86$ & $\pm6.22$ & $\pm6.47$\\ 
\midrule 
Data statistics     & $\pm0.80$ & $\pm0.75$ & $\pm0.69$ & $\pm0.62$ & $\pm0.57$ & $\pm0.53$\\ 
\midrule 
Total uncertainty   & $\pm5.64$ & $\pm6.52$ & $\pm6.00$ & $\pm5.89$ & $\pm6.25$ & $\pm6.49$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_parton_absolute_6bins}
\end{table}


==> tables/systematics_dphi_ll_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.1  &  0.1 -- 0.2  &  0.2 -- 0.3  &  0.3 -- 0.4  &  0.4 -- 0.5  &  0.5 -- 0.6  &  0.6 -- 0.7  &  0.7 -- 0.8  &  0.8 -- 0.9  &  0.9 -- 1.0 \\ 
\midrule 
Source & \multicolumn{10}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.08$ & $\pm 0.37$ & $\pm 1.68$ & $\pm 0.45$ & $\pm 0.42$ & $\pm 1.67$ & $\pm 0.64$ & $\pm 0.37$ & $\pm 0.25$ & $\pm 0.43$\\ 
Parton Distribution Function & $\pm 0.28$ & $\pm 0.29$ & $\pm 0.26$ & $\pm 0.21$ & $\pm 0.12$ & $\pm 0.04$ & $\pm 0.06$ & $\pm 0.18$ & $\pm 0.28$ & $\pm 0.36$\\ 
Parton Shower and Hadronisation & $\pm 0.26$ & $\pm 0.45$ & $\pm 0.11$ & $\pm 0.17$ & $\pm 0.05$ & $\pm 0.59$ & $\pm 0.64$ & $\pm 0.59$ & $\pm 0.32$ & $\pm 0.08$\\ 
Radiation and Scale Settings & $\pm 0.46$ & $\pm 0.60$ & $\pm 1.05$ & $\pm 0.36$ & $\pm 0.62$ & $\pm 0.42$ & $\pm 0.57$ & $\pm 0.84$ & $\pm 0.52$ & $\pm 0.76$\\ 
Background Modelling & $\pm 0.16$ & $\pm 0.21$ & $\pm 0.17$ & $\pm 0.39$ & $\pm 0.17$ & $\pm 0.14$ & $\pm 0.11$ & $\pm 0.19$ & $\pm 0.12$ & $\pm 0.14$\\ 
Pile-up Effects & $\pm 0.08$ & $\pm 0.30$ & $\pm 0.29$ & $\pm 0.11$ & $\pm 0.03$ & $\pm 0.27$ & $\pm 0.11$ & $\pm 0.07$ & $ 0.0 $ & $\pm 0.29$\\ 
Luminosity & $\pm 0.01$ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.09$ & $\pm 0.12$ & $\pm 0.10$ & $\pm 0.08$ & $\pm 0.07$ & $\pm 0.06$ & $\pm 0.02$ & $\pm 0.06$ & $\pm 0.13$ & $\pm 0.15$\\ 
Jet Identification and Reconstruction & $\pm 0.26$ & $\pm 0.27$ & $\pm 0.46$ & $\pm 0.24$ & $\pm 0.24$ & $\pm 0.12$ & $\pm 0.14$ & $\pm 0.18$ & $\pm 0.16$ & $\pm 0.24$\\ 
$b$-tagging & $\pm 0.06$ & $\pm 0.04$ & $\pm 0.05$ & $\pm 0.04$ & $\pm 0.03$ & $\pm 0.03$ & $\pm 0.02$ & $\pm 0.04$ & $\pm 0.04$ & $\pm 0.05$\\ 
Missing Transverse Energy Reconstruction & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.37$ & $\pm 0.36$ & $\pm 0.34$ & $\pm 0.32$ & $\pm 0.31$ & $\pm 0.28$ & $\pm 0.27$ & $\pm 0.25$ & $\pm 0.24$ & $\pm 0.24$\\ 
\midrule 
Total systematics   & $\pm0.84$ & $\pm1.07$ & $\pm2.12$ & $\pm0.88$ & $\pm0.88$ & $\pm1.87$ & $\pm1.13$ & $\pm1.17$ & $\pm0.81$ & $\pm1.08$\\ 
\midrule 
Data statistics     & $\pm1.00$ & $\pm0.94$ & $\pm0.93$ & $\pm0.88$ & $\pm0.83$ & $\pm0.79$ & $\pm0.74$ & $\pm0.70$ & $\pm0.67$ & $\pm0.65$\\ 
\midrule 
Total uncertainty   & $\pm1.30$ & $\pm1.42$ & $\pm2.31$ & $\pm1.25$ & $\pm1.21$ & $\pm2.03$ & $\pm1.35$ & $\pm1.36$ & $\pm1.05$ & $\pm1.26$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_parton_normalised}
\end{table}


==> tables/systematics_dphi_ll_parton_normalised_6bins.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$/[rad/$\pi$] in 6 bins at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$] &  0.0 -- 0.17  &  0.17 -- 0.33  &  0.33 -- 0.50  &  0.50 -- 0.67  &  0.67 -- 0.83  &  0.83 -- 1.0 \\ 
\midrule 
Source & \multicolumn{6}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.81$ & $\pm 0.09$ & $\pm 0.47$ & $\pm 1.42$ & $\pm 0.06$ & $\pm 0.38$\\ 
Parton Distribution Function & $\pm 0.29$ & $\pm 0.26$ & $\pm 0.15$ & $\pm 0.02$ & $\pm 0.18$ & $\pm 0.33$\\ 
Parton Shower and Hadronisation & $\pm 0.41$ & $\pm 0.54$ & $\pm 0.07$ & $\pm 0.63$ & $\pm 0.11$ & $\pm 0.37$\\ 
Radiation and Scale Settings & $\pm 0.69$ & $\pm 0.71$ & $\pm 0.49$ & $\pm 0.16$ & $\pm 0.70$ & $\pm 0.83$\\ 
Background Modelling & $\pm 0.18$ & $\pm 0.17$ & $\pm 0.09$ & $\pm 0.10$ & $\pm 0.05$ & $\pm 0.26$\\ 
Pileup Effects & $\pm 0.11$ & $\pm 0.35$ & $\pm 0.04$ & $\pm 0.11$ & $\pm 0.14$ & $\pm 0.21$\\ 
Luminosity & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.09$ & $\pm 0.09$ & $\pm 0.07$ & $\pm 0.04$ & $\pm 0.05$ & $\pm 0.14$\\ 
Jet Identification and Reconstruction & $\pm 0.28$ & $\pm 0.34$ & $\pm 0.11$ & $\pm 0.07$ & $\pm 0.20$ & $\pm 0.16$\\ 
$b$-tagging & $\pm 0.05$ & $\pm 0.05$ & $\pm 0.02$ & $\pm 0.02$ & $\pm 0.03$ & $\pm 0.05$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $ & $\pm 0.0 $\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.27$ & $\pm 0.26$ & $\pm 0.23$ & $\pm 0.21$ & $\pm 0.19$ & $\pm 0.18$\\ 
\midrule 
Total systematics   & $\pm1.26$ & $\pm1.10$ & $\pm0.76$ & $\pm1.58$ & $\pm0.80$ & $\pm1.13$\\ 
\midrule 
Data statistics     & $\pm0.72$ & $\pm0.69$ & $\pm0.63$ & $\pm0.57$ & $\pm0.52$ & $\pm0.49$\\ 
\midrule 
Total uncertainty   & $\pm1.45$ & $\pm1.30$ & $\pm0.98$ & $\pm1.68$ & $\pm0.96$ & $\pm1.24$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_parton_normalised_6bins}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_450_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} < 450$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} < 450$ GeV       & 0.0 -- 0.2  &  0.2 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0 \\\midrule 
Source & \multicolumn{5}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 5.16$ & $\pm 3.51$ & $\pm 4.48$ & $\pm 4.67$ & $\pm 4.22$\\ 
Parton Distribution Function & $\pm 1.16$ & $\pm 1.17$ & $\pm 1.15$ & $\pm 1.17$ & $\pm 1.14$\\ 
Parton Shower and Hadronisation & $\pm 0.64$ & $\pm 1.59$ & $\pm 0.83$ & $\pm 0.16$ & $\pm 2.52$\\ 
Radiation and Scale Settings & $\pm 0.79$ & $\pm 0.84$ & $\pm 0.9$ & $\pm 0.36$ & $\pm 0.39$\\ 
Background Modelling & $\pm 0.3$ & $\pm 0.41$ & $\pm 0.43$ & $\pm 0.39$ & $\pm 0.63$\\ 
Pile-up Effects & $\pm 1.89$ & $\pm 1.51$ & $\pm 1.97$ & $\pm 1.53$ & $\pm 1.61$\\ 
Luminosity & $\pm 2.16$ & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.18$\\ 
Lepton Identification and Reconstruction & $\pm 1.23$ & $\pm 1.21$ & $\pm 1.19$ & $\pm 1.14$ & $\pm 1.29$\\ 
Jet Identification and Reconstruction & $\pm 3.26$ & $\pm 3.78$ & $\pm 3.16$ & $\pm 3.75$ & $\pm 2.78$\\ 
$b$-tagging & $\pm 4.7$ & $\pm 4.76$ & $\pm 4.88$ & $\pm 5.05$ & $\pm 5.09$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.61$ & $\pm 0.7$ & $\pm 1.25$ & $\pm 0.48$ & $\pm 1.48$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.58$ & $\pm 0.59$ & $\pm 0.55$ & $\pm 0.56$ & $\pm 0.57$\\ 
\midrule 
Total systematics   & $\pm8.5$ & $\pm7.96$ & $\pm8.29$ & $\pm8.48$ & $\pm8.61$\\ 
\midrule 
Data statistics     & $\pm1.67$ & $\pm1.68$ & $\pm1.64$ & $\pm1.6$ & $\pm1.7$\\ 
\midrule 
Total uncertainty   & $\pm8.66$ & $\pm8.14$ & $\pm8.45$ & $\pm8.63$ & $\pm8.77$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_450_particle_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_450_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} < 450$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_450_particle_normalised}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} < 450$ GeV       & 0.0 -- 0.2  &  0.2 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0 \\\midrule 
Source & \multicolumn{5}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.76$ & $\pm 0.89$ & $\pm 0.15$ & $\pm 0.26$ & $\pm 0.27$\\ 
Parton Distribution Function & $\pm 0.06$ & $\pm 0.05$ & $\pm 0.02$ & $\pm 0.04$ & $\pm 0.09$\\ 
Parton Shower and Hadronisation & $\pm 0.17$ & $\pm 2.04$ & $\pm 0.34$ & $\pm 0.33$ & $\pm 2.00$\\ 
Radiation and Scale Settings & $\pm 0.64$ & $\pm 0.70$ & $\pm 1.03$ & $\pm 0.22$ & $\pm 0.53$\\ 
Background Modelling & $\pm 0.27$ & $\pm 0.05$ & $\pm 0.06$ & $\pm 0.08$ & $\pm 0.26$\\ 
Pile-up Effects & $\pm 0.19$ & $\pm 0.20$ & $\pm 0.27$ & $\pm 0.17$ & $\pm 0.09$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.59$ & $\pm 0.60$ & $\pm 0.59$ & $\pm 0.53$ & $\pm 0.66$\\ 
Jet Identification and Reconstruction & $\pm 1.14$ & $\pm 2.10$ & $\pm 1.65$ & $\pm 1.61$ & $\pm 2.03$\\ 
$b$-tagging & $\pm 0.24$ & $\pm 0.16$ & $\pm 0.05$ & $\pm 0.20$ & $\pm 0.24$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.61$ & $\pm 0.42$ & $\pm 0.72$ & $\pm 0.77$ & $\pm 0.87$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.60$ & $\pm 0.60$ & $\pm 0.53$ & $\pm 0.55$ & $\pm 0.58$\\ 
\midrule 
Total systematics   & $\pm1.88$ & $\pm3.29$ & $\pm2.27$ & $\pm2.02$ & $\pm3.19$\\ 
\midrule 
Data statistics     & $\pm1.48$ & $\pm1.49$ & $\pm1.46$ & $\pm1.44$ & $\pm1.55$\\ 
\midrule 
Total uncertainty   & $\pm2.40$ & $\pm3.61$ & $\pm2.70$ & $\pm2.48$ & $\pm3.54$\\ 
\bottomrule 
\end{tabular}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_450_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} < 450$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} < 450$ GeV       & 0.0 -- 0.2  &  0.2 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0 \\\midrule 
Source & \multicolumn{5}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 4.16$ & $\pm 3.52$ & $\pm 3.42$ & $\pm 1.47$ & $\pm 0.92$\\ 
Parton Distribution Function & $\pm 1.17$ & $\pm 1.18$ & $\pm 1.16$ & $\pm 1.18$ & $\pm 1.16$\\ 
Parton Shower and Hadronisation & $\pm 0.11$ & $\pm 2.36$ & $\pm 0.97$ & $\pm 2.22$ & $\pm 1.33$\\ 
Radiation and Scale Settings & $\pm 1.29$ & $\pm 0.56$ & $\pm 1.8$ & $\pm 0.04$ & $\pm 1.65$\\ 
Background Modelling & $\pm 0.3$ & $\pm 0.41$ & $\pm 0.43$ & $\pm 0.39$ & $\pm 0.64$\\ 
Pile-up Effects & $\pm 1.89$ & $\pm 1.5$ & $\pm 1.98$ & $\pm 1.54$ & $\pm 1.62$\\ 
Luminosity & $\pm 2.16$ & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.18$\\ 
Lepton Identification and Reconstruction & $\pm 1.25$ & $\pm 1.21$ & $\pm 1.2$ & $\pm 1.16$ & $\pm 1.31$\\ 
Jet Identification and Reconstruction & $\pm 3.28$ & $\pm 3.83$ & $\pm 3.21$ & $\pm 3.84$ & $\pm 2.85$\\ 
$b$-tagging & $\pm 4.71$ & $\pm 4.77$ & $\pm 4.89$ & $\pm 5.06$ & $\pm 5.1$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.62$ & $\pm 0.71$ & $\pm 1.3$ & $\pm 0.5$ & $\pm 1.54$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.6$ & $\pm 0.61$ & $\pm 0.57$ & $\pm 0.58$ & $\pm 0.6$\\ 
\midrule 
Total systematics   & $\pm7.99$ & $\pm8.16$ & $\pm7.98$ & $\pm7.62$ & $\pm7.49$\\ 
\midrule 
Data statistics     & $\pm1.62$ & $\pm1.64$ & $\pm1.6$ & $\pm1.58$ & $\pm1.67$\\ 
\midrule 
Total uncertainty   & $\pm8.16$ & $\pm8.32$ & $\pm8.14$ & $\pm7.78$ & $\pm7.67$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_450_parton_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_450_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} < 450$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} < 450$ GeV       & 0.0 -- 0.2  &  0.2 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0 \\\midrule 
Source & \multicolumn{5}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.73$ & $\pm 1.07$ & $\pm 1.02$ & $\pm 0.99$ & $\pm 3.43$\\ 
Parton Distribution Function & $\pm 0.06$ & $\pm 0.05$ & $\pm 0.02$ & $\pm 0.04$ & $\pm 0.09$\\ 
Parton Shower and Hadronisation & $\pm 1.41$ & $\pm 1.02$ & $\pm 0.36$ & $\pm 0.86$ & $\pm 0.02$\\ 
Radiation and Scale Settings & $\pm 1.55$ & $\pm 0.83$ & $\pm 1.50$ & $\pm 0.24$ & $\pm 1.36$\\ 
Background Modelling & $\pm 0.27$ & $\pm 0.06$ & $\pm 0.07$ & $\pm 0.08$ & $\pm 0.28$\\ 
Pile-up Effects & $\pm 0.18$ & $\pm 0.21$ & $\pm 0.27$ & $\pm 0.17$ & $\pm 0.09$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.60$ & $\pm 0.62$ & $\pm 0.62$ & $\pm 0.57$ & $\pm 0.71$\\ 
Jet Identification and Reconstruction & $\pm 1.16$ & $\pm 2.14$ & $\pm 1.72$ & $\pm 1.73$ & $\pm 2.17$\\ 
$b$-tagging & $\pm 0.24$ & $\pm 0.16$ & $\pm 0.05$ & $\pm 0.22$ & $\pm 0.26$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.61$ & $\pm 0.42$ & $\pm 0.77$ & $\pm 0.80$ & $\pm 0.93$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.60$ & $\pm 0.62$ & $\pm 0.55$ & $\pm 0.57$ & $\pm 0.60$\\ 
\midrule 
Total systematics   & $\pm3.17$ & $\pm2.91$ & $\pm2.78$ & $\pm2.48$ & $\pm4.49$\\ 
\midrule 
Data statistics     & $\pm1.41$ & $\pm1.44$ & $\pm1.43$ & $\pm1.43$ & $\pm1.54$\\ 
\midrule 
Total uncertainty   & $\pm3.47$ & $\pm3.25$ & $\pm3.13$ & $\pm2.86$ & $\pm4.75$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_450_parton_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_550_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $450 < m_{t\bar{t}} < 550$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $450 < m_{t\bar{t}} < 550$ GeV & 0.0 -- 0.3  &  0.3 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 4.16$ & $\pm 3.62$ & $\pm 0.5$ & $\pm 2.36$\\ 
Parton Distribution Function & $\pm 0.85$ & $\pm 0.79$ & $\pm 0.78$ & $\pm 0.79$\\ 
Parton Shower and Hadronisation & $\pm 2.4$ & $\pm 3.03$ & $\pm 2.7$ & $\pm 1.63$\\ 
Radiation and Scale Settings & $\pm 1.8$ & $\pm 0.28$ & $\pm 1.93$ & $\pm 0.85$\\ 
Background Modelling & $\pm 0.37$ & $\pm 0.28$ & $\pm 0.47$ & $\pm 0.5$\\ 
Pile-up Effects & $\pm 2.11$ & $\pm 1.57$ & $\pm 1.35$ & $\pm 1.44$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.16$ & $\pm 2.17$ & $\pm 2.17$\\ 
Lepton Identification and Reconstruction & $\pm 2.49$ & $\pm 1.61$ & $\pm 1.36$ & $\pm 1.29$\\ 
Jet Identification and Reconstruction & $\pm 5.9$ & $\pm 2.73$ & $\pm 2.86$ & $\pm 3.67$\\ 
$b$-tagging & $\pm 4.24$ & $\pm 4.49$ & $\pm 4.65$ & $\pm 4.75$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.06$ & $\pm 0.69$ & $\pm 0.92$ & $\pm 0.73$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.73$ & $\pm 0.53$ & $\pm 0.5$ & $\pm 0.47$\\ 
\midrule 
Total systematics   & $\pm9.85$ & $\pm8.0$ & $\pm7.52$ & $\pm7.42$\\ 
\midrule 
Data statistics     & $\pm2.16$ & $\pm1.51$ & $\pm1.44$ & $\pm1.4$\\ 
\midrule 
Total uncertainty   & $\pm10.08$ & $\pm8.14$ & $\pm7.65$ & $\pm7.55$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_550_particle_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_550_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $450 \leq m_{t\bar{t}} < 550$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $450 \leq m_{t\bar{t}} < 550$ GeV & 0.0 -- 0.3  &  0.3 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 3.41$ & $\pm 2.84$ & $\pm 1.41$ & $\pm 3.35$\\ 
Parton Distribution Function & $\pm 0.10$ & $\pm 0.05$ & $\pm 0.03$ & $\pm 0.09$\\ 
Parton Shower and Hadronisation & $\pm 0.01$ & $\pm 0.63$ & $\pm 0.27$ & $\pm 0.82$\\ 
Radiation and Scale Settings & $\pm 0.67$ & $\pm 0.83$ & $\pm 0.76$ & $\pm 0.29$\\ 
Background Modelling & $\pm 0.07$ & $\pm 0.19$ & $\pm 0.09$ & $\pm 0.13$\\ 
Pile-up Effects & $\pm 0.55$ & $\pm 0.01$ & $\pm 0.21$ & $\pm 0.09$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 2.04$ & $\pm 1.21$ & $\pm 0.73$ & $\pm 0.57$\\ 
Jet Identification and Reconstruction & $\pm 3.96$ & $\pm 1.95$ & $\pm 2.01$ & $\pm 1.50$\\ 
$b$-tagging & $\pm 0.41$ & $\pm 0.09$ & $\pm 0.11$ & $\pm 0.24$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.74$ & $\pm 0.85$ & $\pm 0.75$ & $\pm 0.60$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.92$ & $\pm 0.52$ & $\pm 0.45$ & $\pm 0.40$\\ 
\midrule 
Total systematics   & $\pm5.81$ & $\pm3.94$ & $\pm2.92$ & $\pm3.93$\\ 
\midrule 
Data statistics     & $\pm1.92$ & $\pm1.27$ & $\pm1.28$ & $\pm1.20$\\ 
\midrule 
Total uncertainty   & $\pm6.12$ & $\pm4.14$ & $\pm3.19$ & $\pm4.11$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_550_particle_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_550_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $450 < m_{t\bar{t}} < 550$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $450 < m_{t\bar{t}} < 550$ GeV & 0.0 -- 0.3  &  0.3 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 5.48$ & $\pm 4.28$ & $\pm 6.22$ & $\pm 6.15$\\ 
Parton Distribution Function & $\pm 0.86$ & $\pm 0.8$ & $\pm 0.8$ & $\pm 0.82$\\ 
Parton Shower and Hadronisation & $\pm 0.63$ & $\pm 1.07$ & $\pm 1.1$ & $\pm 0.93$\\ 
Radiation and Scale Settings & $\pm 0.77$ & $\pm 0.55$ & $\pm 2.44$ & $\pm 1.24$\\ 
Background Modelling & $\pm 0.37$ & $\pm 0.28$ & $\pm 0.47$ & $\pm 0.51$\\ 
Pile-up Effects & $\pm 2.09$ & $\pm 1.58$ & $\pm 1.37$ & $\pm 1.46$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.16$ & $\pm 2.17$ & $\pm 2.17$\\ 
Lepton Identification and Reconstruction & $\pm 2.37$ & $\pm 1.57$ & $\pm 1.34$ & $\pm 1.27$\\ 
Jet Identification and Reconstruction & $\pm 5.69$ & $\pm 2.68$ & $\pm 2.88$ & $\pm 3.58$\\ 
$b$-tagging & $\pm 4.26$ & $\pm 4.51$ & $\pm 4.67$ & $\pm 4.76$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.02$ & $\pm 0.66$ & $\pm 0.9$ & $\pm 0.76$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.69$ & $\pm 0.51$ & $\pm 0.49$ & $\pm 0.46$\\ 
\midrule 
Total systematics   & $\pm9.93$ & $\pm7.81$ & $\pm9.55$ & $\pm9.27$\\ 
\midrule 
Data statistics     & $\pm1.92$ & $\pm1.39$ & $\pm1.35$ & $\pm1.31$\\ 
\midrule 
Total uncertainty   & $\pm10.11$ & $\pm7.94$ & $\pm9.64$ & $\pm9.36$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_550_parton_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_550_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $450 \leq m_{t\bar{t}} < 550$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $450 \leq m_{t\bar{t}} < 550$ GeV & 0.0 -- 0.3  &  0.3 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.04$ & $\pm 1.22$ & $\pm 0.82$ & $\pm 0.67$\\ 
Parton Distribution Function & $\pm 0.09$ & $\pm 0.05$ & $\pm 0.04$ & $\pm 0.10$\\ 
Parton Shower and Hadronisation & $\pm 0.30$ & $\pm 0.13$ & $\pm 0.16$ & $\pm 0.02$\\ 
Radiation and Scale Settings & $\pm 0.12$ & $\pm 1.42$ & $\pm 1.52$ & $\pm 0.34$\\ 
Background Modelling & $\pm 0.06$ & $\pm 0.17$ & $\pm 0.11$ & $\pm 0.15$\\ 
Pile-up Effects & $\pm 0.48$ & $\pm 0.12$ & $\pm 0.26$ & $\pm 0.17$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 1.80$ & $\pm 1.24$ & $\pm 0.79$ & $\pm 0.56$\\ 
Jet Identification and Reconstruction & $\pm 3.52$ & $\pm 2.02$ & $\pm 2.07$ & $\pm 1.45$\\ 
$b$-tagging & $\pm 0.36$ & $\pm 0.06$ & $\pm 0.15$ & $\pm 0.28$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.63$ & $\pm 0.78$ & $\pm 0.74$ & $\pm 0.64$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.85$ & $\pm 0.49$ & $\pm 0.44$ & $\pm 0.39$\\ 
\midrule 
Total systematics   & $\pm4.15$ & $\pm3.17$ & $\pm3.03$ & $\pm1.99$\\ 
\midrule 
Data statistics     & $\pm1.59$ & $\pm1.17$ & $\pm1.25$ & $\pm1.20$\\ 
\midrule 
Total uncertainty   & $\pm4.45$ & $\pm3.38$ & $\pm3.28$ & $\pm2.32$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_550_parton_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_800_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $550 < m_{t\bar{t}} < 800$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $550 < m_{t\bar{t}} < 800$ GeV & 0.0 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.97$ & $\pm 2.56$ & $\pm 2.17$ & $\pm 0.64$\\ 
Parton Distribution Function & $\pm 0.91$ & $\pm 0.73$ & $\pm 0.71$ & $\pm 0.64$\\ 
Parton Shower and Hadronisation & $\pm 2.28$ & $\pm 2.77$ & $\pm 4.82$ & $\pm 3.49$\\ 
Radiation and Scale Settings & $\pm 1.13$ & $\pm 4.52$ & $\pm 2.07$ & $\pm 0.56$\\ 
Background Modelling & $\pm 0.42$ & $\pm 0.44$ & $\pm 0.34$ & $\pm 0.4$\\ 
Pile-up Effects & $\pm 1.45$ & $\pm 1.69$ & $\pm 1.04$ & $\pm 1.02$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.16$ & $\pm 2.16$\\ 
Lepton Identification and Reconstruction & $\pm 2.06$ & $\pm 1.34$ & $\pm 1.44$ & $\pm 1.45$\\ 
Jet Identification and Reconstruction & $\pm 4.8$ & $\pm 3.85$ & $\pm 2.47$ & $\pm 2.49$\\ 
$b$-tagging & $\pm 4.1$ & $\pm 4.31$ & $\pm 4.37$ & $\pm 4.44$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.17$ & $\pm 1.66$ & $\pm 0.68$ & $\pm 1.14$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.97$ & $\pm 0.89$ & $\pm 0.63$ & $\pm 0.51$\\ 
\midrule 
Total systematics   & $\pm8.39$ & $\pm9.04$ & $\pm8.32$ & $\pm7.0$\\ 
\midrule 
Data statistics     & $\pm2.8$ & $\pm2.57$ & $\pm1.81$ & $\pm1.51$\\ 
\midrule 
Total uncertainty   & $\pm8.85$ & $\pm9.4$ & $\pm8.51$ & $\pm7.16$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_800_particle_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_800_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $550 \leq m_{t\bar{t}} < 800$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $550 \leq m_{t\bar{t}} < 800$ GeV & 0.0 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.80$ & $\pm 2.47$ & $\pm 2.52$ & $\pm 0.45$\\ 
Parton Distribution Function & $\pm 0.28$ & $\pm 0.07$ & $\pm 0.04$ & $\pm 0.13$\\ 
Parton Shower and Hadronisation & $\pm 1.26$ & $\pm 0.74$ & $\pm 1.26$ & $\pm 0.07$\\ 
Radiation and Scale Settings & $\pm 0.58$ & $\pm 3.99$ & $\pm 2.66$ & $\pm 0.01$\\ 
Background Modelling & $\pm 0.11$ & $\pm 0.14$ & $\pm 0.06$ & $\pm 0.02$\\ 
Pile-up Effects & $\pm 0.24$ & $\pm 0.49$ & $\pm 0.05$ & $\pm 0.34$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 1.31$ & $\pm 0.89$ & $\pm 0.69$ & $\pm 0.39$\\ 
Jet Identification and Reconstruction & $\pm 3.14$ & $\pm 2.41$ & $\pm 2.02$ & $\pm 1.21$\\ 
$b$-tagging & $\pm 0.31$ & $\pm 0.09$ & $\pm 0.05$ & $\pm 0.12$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.39$ & $\pm 1.42$ & $\pm 0.94$ & $\pm 0.94$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.26$ & $\pm 1.10$ & $\pm 0.58$ & $\pm 0.33$\\ 
\midrule 
Total systematics   & $\pm4.52$ & $\pm5.71$ & $\pm4.57$ & $\pm1.72$\\ 
\midrule 
Data statistics     & $\pm2.49$ & $\pm2.30$ & $\pm1.55$ & $\pm1.26$\\ 
\midrule 
Total uncertainty   & $\pm5.16$ & $\pm6.16$ & $\pm4.83$ & $\pm2.13$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_800_particle_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_800_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $550 < m_{t\bar{t}} < 800$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $550 < m_{t\bar{t}} < 800$ GeV & 0.0 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 7.6$ & $\pm 8.02$ & $\pm 6.5$ & $\pm 7.75$\\ 
Parton Distribution Function & $\pm 0.9$ & $\pm 0.72$ & $\pm 0.7$ & $\pm 0.63$\\ 
Parton Shower and Hadronisation & $\pm 1.28$ & $\pm 0.01$ & $\pm 2.27$ & $\pm 0.58$\\ 
Radiation and Scale Settings & $\pm 1.07$ & $\pm 4.7$ & $\pm 2.71$ & $\pm 0.18$\\ 
Background Modelling & $\pm 0.41$ & $\pm 0.44$ & $\pm 0.34$ & $\pm 0.4$\\ 
Pile-up Effects & $\pm 1.46$ & $\pm 1.69$ & $\pm 1.05$ & $\pm 1.03$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.17$ & $\pm 2.16$ & $\pm 2.16$\\ 
Lepton Identification and Reconstruction & $\pm 2.02$ & $\pm 1.32$ & $\pm 1.43$ & $\pm 1.44$\\ 
Jet Identification and Reconstruction & $\pm 4.79$ & $\pm 3.81$ & $\pm 2.55$ & $\pm 2.51$\\ 
$b$-tagging & $\pm 4.1$ & $\pm 4.32$ & $\pm 4.38$ & $\pm 4.44$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.14$ & $\pm 1.62$ & $\pm 0.67$ & $\pm 1.11$\\ 
Monte Carlo Statistical Uncertainty & $\pm 0.94$ & $\pm 0.85$ & $\pm 0.62$ & $\pm 0.5$\\ 
\midrule 
Total systematics   & $\pm11.08$ & $\pm11.53$ & $\pm9.57$ & $\pm9.82$\\ 
\midrule 
Data statistics     & $\pm2.57$ & $\pm2.38$ & $\pm1.69$ & $\pm1.42$\\ 
\midrule 
Total uncertainty   & $\pm11.37$ & $\pm11.77$ & $\pm9.72$ & $\pm9.92$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_800_parton_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_m_800_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $550 \leq m_{t\bar{t}} < 800$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $550 \leq m_{t\bar{t}} < 800$ GeV & 0.0 -- 0.4  &  0.4 -- 0.6  &  0.6 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{4}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.10$ & $\pm 0.47$ & $\pm 0.98$ & $\pm 0.42$\\ 
Parton Distribution Function & $\pm 0.24$ & $\pm 0.04$ & $\pm 0.07$ & $\pm 0.17$\\ 
Parton Shower and Hadronisation & $\pm 0.22$ & $\pm 1.07$ & $\pm 1.18$ & $\pm 0.50$\\ 
Radiation and Scale Settings & $\pm 0.57$ & $\pm 4.24$ & $\pm 3.25$ & $\pm 0.34$\\ 
Background Modelling & $\pm 0.10$ & $\pm 0.14$ & $\pm 0.05$ & $\pm 0.02$\\ 
Pile-up Effects & $\pm 0.20$ & $\pm 0.43$ & $\pm 0.13$ & $\pm 0.41$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $ & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 1.14$ & $\pm 0.87$ & $\pm 0.80$ & $\pm 0.50$\\ 
Jet Identification and Reconstruction & $\pm 2.70$ & $\pm 2.22$ & $\pm 2.27$ & $\pm 1.47$\\ 
$b$-tagging & $\pm 0.27$ & $\pm 0.08$ & $\pm 0.09$ & $\pm 0.16$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.20$ & $\pm 1.43$ & $\pm 0.81$ & $\pm 1.08$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.18$ & $\pm 1.00$ & $\pm 0.53$ & $\pm 0.29$\\ 
\midrule 
Total systematics   & $\pm3.73$ & $\pm5.32$ & $\pm4.46$ & $\pm2.10$\\ 
\midrule 
Data statistics     & $\pm2.03$ & $\pm2.14$ & $\pm1.57$ & $\pm1.35$\\ 
\midrule 
Total uncertainty   & $\pm4.24$ & $\pm5.73$ & $\pm4.73$ & $\pm2.50$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_m_800_parton_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_max_particle_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} > 800$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c }
\toprule
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} > 800$ GeV       & 0.0 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{2}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 1.11$ & $\pm 4.29$\\ 
Parton Distribution Function & $\pm 1.82$ & $\pm 1.83$\\ 
Parton Shower and Hadronisation & $\pm 10.55$ & $\pm 5.89$\\ 
Radiation and Scale Settings & $\pm 1.44$ & $\pm 1.49$\\ 
Background Modelling & $\pm 0.71$ & $\pm 0.47$\\ 
Pile-up Effects & $\pm 1.51$ & $\pm 0.46$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.16$\\ 
Lepton Identification and Reconstruction & $\pm 1.86$ & $\pm 2.61$\\ 
Jet Identification and Reconstruction & $\pm 3.4$ & $\pm 5.62$\\ 
$b$-tagging & $\pm 4.4$ & $\pm 4.46$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.68$ & $\pm 3.34$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.03$ & $\pm 0.95$\\ 
\midrule 
Total systematics   & $\pm12.73$ & $\pm11.61$\\ 
\midrule 
Data statistics     & $\pm3.01$ & $\pm2.83$\\ 
\midrule 
Total uncertainty   & $\pm13.08$ & $\pm11.95$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_max_particle_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_max_particle_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} \geq 800$ GeV at particle level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} \geq 800$ GeV       & 0.0 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{2}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 2.87$ & $\pm 2.91$\\ 
Parton Distribution Function & $\pm 0.22$ & $\pm 0.22$\\ 
Parton Shower and Hadronisation & $\pm 2.23$ & $\pm 2.25$\\ 
Radiation and Scale Settings & $ 0.0 $ & $ 0.0 $\\ 
Background Modelling & $\pm 0.14$ & $\pm 0.14$\\ 
Pile-up Effects & $\pm 0.82$ & $\pm 0.37$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 1.03$ & $\pm 1.01$\\ 
Jet Identification and Reconstruction & $\pm 2.73$ & $\pm 3.07$\\ 
$b$-tagging & $\pm 0.09$ & $\pm 0.09$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.58$ & $\pm 1.60$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.07$ & $\pm 0.91$\\ 
\midrule 
Total systematics   & $\pm5.22$ & $\pm5.25$\\ 
\midrule 
Data statistics     & $\pm2.01$ & $\pm2.13$\\ 
\midrule 
Total uncertainty   & $\pm5.59$ & $\pm5.66$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_max_particle_normalised}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_max_parton_absolute.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the absolute differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} > 800$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 correspond to uncertainties smaller than 0.005 in magnitude. Asymmetric systematic uncertainties have been symmetrised for this summary table.}
\vspace{3mm}
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} > 800$ GeV       & 0.0 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{2}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 7.96$ & $\pm 6.36$\\ 
Parton Distribution Function & $\pm 1.82$ & $\pm 1.82$\\ 
Parton Shower and Hadronisation & $\pm 6.89$ & $\pm 1.27$\\ 
Radiation and Scale Settings & $\pm 1.29$ & $\pm 1.45$\\ 
Background Modelling & $\pm 0.71$ & $\pm 0.47$\\ 
Pile-up Effects & $\pm 1.51$ & $\pm 0.46$\\ 
Luminosity & $\pm 2.17$ & $\pm 2.16$\\ 
Lepton Identification and Reconstruction & $\pm 1.85$ & $\pm 2.6$\\ 
Jet Identification and Reconstruction & $\pm 3.38$ & $\pm 5.58$\\ 
$b$-tagging & $\pm 4.4$ & $\pm 4.46$\\ 
Missing Transverse Energy Reconstruction & $\pm 0.68$ & $\pm 3.32$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.02$ & $\pm 0.95$\\ 
\midrule 
Total systematics   & $\pm12.64$ & $\pm11.09$\\ 
\midrule 
Data statistics     & $\pm2.84$ & $\pm2.69$\\ 
\midrule 
Total uncertainty   & $\pm12.95$ & $\pm11.41$\\ 
\bottomrule 
\end{tabular}
\label{tab:syst_small_dphi_ll_vs_ttbar_max_parton_absolute}
\end{table}


==> tables/systematics_dphi_ll_vs_ttbar_max_parton_normalised.tex <==
\begin{table}
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})$ in the region $m_{t\bar{t}} \geq 800$ GeV at parton level, presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.005 in magnitude. Any asymmetric systematic uncertainties have been symmetrised for this summary table.}
\label{tab:syst_small_dphi_ll_vs_ttbar_max_parton_normalised}
\scriptsize
\scriptsize
\centering
\setlength\extrarowheight{6pt}
\begin{tabular}{l  c  c }
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})$ [rad/$\pi$], $m_{t\bar{t}} \geq 800$ GeV       & 0.0 -- 0.8  &  0.8 -- 1.0  \\\midrule 
Source & \multicolumn{2}{c}{ Systematic uncertainty (\%) } \\ 
\midrule 
Matrix Element & $\pm 0.48$ & $\pm 0.73$\\ 
Parton Distribution Function & $\pm 0.18$ & $\pm 0.27$\\ 
Parton Shower and Hadronisation & $\pm 2.13$ & $\pm 3.26$\\ 
Radiation and Scale Settings & $\pm 0.05$ & $\pm 0.08$\\ 
Background Modelling & $\pm 0.11$ & $\pm 0.17$\\ 
Pile-up Effects & $\pm 0.65$ & $\pm 0.45$\\ 
Luminosity & $ 0.0 $ & $ 0.0 $\\ 
Lepton Identification and Reconstruction & $\pm 0.81$ & $\pm 1.21$\\ 
Jet Identification and Reconstruction & $\pm 2.15$ & $\pm 3.66$\\ 
$b$-tagging & $\pm 0.07$ & $\pm 0.11$\\ 
Missing Transverse Energy Reconstruction & $\pm 1.24$ & $\pm 1.89$\\ 
Monte Carlo Statistical Uncertainty & $\pm 1.05$ & $\pm 0.90$\\ 
\midrule 
Total systematics   & $\pm3.72$ & $\pm5.55$\\ 
\midrule 
Data statistics     & $\pm1.50$ & $\pm2.41$\\ 
\midrule 
Total uncertainty   & $\pm4.01$ & $\pm6.05$\\ 
\bottomrule 
\end{tabular}
\end{table}


==> tables/systematics_full_dphi_ll_parton_normalised.tex <==
\tiny
\begin{longtable}{l  c  c  c  c  c  c  c  c  c  c }
\caption{Summary of the sources of uncertainty on the normalised differential cross section for $\Delta\phi(\ell^{+},\ell^{-})/\pi$ at parton level. The uncertainties are presented as a percentage of the measured cross-section in each bin. Entries with 0.0 are uncertainties that are less than 0.05 in magnitude. For systematics that have only one variation, $\pm$($\mp$) indicates that the systematic shift was positive (negative) and then symmetrised. The $b$-tagging systematics have been broken down into separate $b$-quark (B), $c$-quark (C), and light quark eigenvector components.}
\label{tab:syst_full_dphi_ll_parton_normalised}
\toprule 
$\Delta\phi(\ell^{+},\ell^{-})/\pi$: normalised & $0.0$ - $0.1$ & $0.1$ - $0.2$ & $0.2$ - $0.3$ & $0.3$ - $0.4$ & $0.4$ - $0.5$ & $0.5$ - $0.6$ & $0.6$ - $0.7$ & $0.7$ - $0.8$ & $0.8$ - $0.9$ & $0.9$ - $1.0$\\
\midrule 
\bottomrule 

\end{longtable}

